Atlas: Hierarchical Partitioning for Quantum Circuit Simulation on GPUs (Extended Version)

This paper presents techniques for theoretically and practically efficient and scalable Schr\"odinger-style quantum circuit simulation. Our approach partitions a quantum circuit into a hierarchy of subcircuits and simulates the subcircuits on multi-node GPUs, exploiting available data parallelism while minimizing communication costs. To minimize communication costs, we formulate an Integer Linear Program that rewards simulation of "nearby" gates on "nearby" GPUs. To maximize throughput, we use a dynamic programming algorithm to compute the subcircuit simulated by each kernel at a GPU. We realize these techniques in Atlas, a distributed, multi-GPU quantum circuit simulator. Our evaluation on a variety of quantum circuits shows that Atlas outperforms state-of-the-art GPU-based simulators by more than 2$\times$ on average and is able to run larger circuits via offloading to DRAM, outperforming other large-circuit simulators by two orders of magnitude.

==> approach.tex <==
\section{Overview of \Sys}
\label{sec:overview}

TODO: STALE. BLEND.

\begin{algorithm}[tb]
\small
\begin{algorithmic}[1]
\Function{Simulate}{$\m{C},l,o, state$}
\State $(\m{C}_0,\m{M}_0),\dots,(\m{C}_{s-1},\m{M}_{s-1}) = \Call{Partition}{\m{C},l,o}$
\State // The initial state vector is mapped by $\m{M}_0$.
%\State $(\m{K}_{0,0},\dots,\m{K}_{0,b_0-1}),\dots,(\m{K}_{s-1,0},\dots,\m{K}_{0,b_{s-1}-1}) = \Call{Preprocess}{\m{C},l,o}$
\For{$i=0,\dots,s-1$}
\If {$i > 0$}
\State $state = \Call{RemapQubits}{state, \m{M}_{i-1},\m{M}_i}$
\EndIf
\State $\m{K}_{0},\dots,\m{K}_{b-1} = \Call{Kernelize}{\m{C}_i}$
\For{$j=0,\dots,b-1$}
\State $state = \Call{LaunchKernel}{state, \m{K}_j}$
\EndFor
\EndFor
\State \Return $state$
\EndFunction
%\Function{Preprocess}{$\m{C},l,o$}
%\State $(\m{C}_0,\m{M}_0),\dots,(\m{C}_{s-1},\m{M}_{s-1}) = \Call{Partition}{\m{C},l,o}$
%\State \Return $\Call{Kernelize}{\m{C}_0},\dots,\Call{Kernelize}{\m{C}_{s-1}}$
%\EndFunction
\end{algorithmic}
%\vspace{-0.5em}
\caption{An overview of \Syss circuit simulation algorithm, simulating a circuit $\m{C}$ on the input $state$ with $l$ local qubits and $o$ global qubits.}%\vspace{-0.5em}}
%\label{alg:overview}
\end{algorithm}

\if 0
\begin{figure}
    \centering
    \includegraphics[scale=0.42]{figures/dnn_parallelization.pdf}
    \caption{Data and pipeline parallelism for DNN training. Green arrows indicate communications between GPUs.}
    \label{fig:dnn_parallelization}
\end{figure}
\fi 

\begin{figure}
%\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.3]{figures/qcs_to_dnn_translation.pdf}
    %\vspace{-1em}
    \caption{Transforming a 3-qubit quantum circuit to a DNN computation graph that takes as input a 2$\times$2$\times$2 tensor. The weights for the three linear layers (i.e., $U_H$, $U_{CX}$, and $U_{CU}$) are the unitary matrices of the three quantum gates.}
    \label{fig:qcs_to_dnn_transformation}
%\end{wrapfigure}
\end{figure}
\if 0
\UA{Replaced by paras below by merging from prior section}
A key idea behind \Sys is transforming quantum circuit simulation to DNN computation, which allows \Sys to perform distributed simulation on existing DNN frameworks. 
%%%
In particular, the state vector of an $n$-qubit quantum system can be represented as a tensor with $n$ dimensions, each of which has a size of two. Therefore, the overall number of elements in this tensor is $2^n$. 
%%%
A quantum circuit manipulates the state vector by applying gates to one or multiple qubits. Each quantum gate can be considered as a linear transformation to the corresponding dimensions, whose weights are given by the unitary matrix of the gate. 
%%%
\fi

Both deep neural networks (DNNs) and quantum circuit simulation revolve around tensor algebra computations.
%
%Much like a quantum circuit (a graph), a DNN is also represented as a computation graph, where each node is a tensor operator such as matrix multiplication or convolution and each edge is a tensor (i.e., $n$-dimensional array) shared between operators.
%
A key idea behind \Sys is transforming a quantum circuit to a DNN computation graph, which allows \Sys to perform distributed simulation on existing DNN frameworks.
In particular, the state vector over $n$-qubits can be represented as a tensor with $n$ dimensions, each of which has a size of two, leading to an overall tensor size of $2^n$.
A quantum circuit manipulates the state vector by applying gates to qubits. 
Each quantum gate can be considered as a linear transformation to the corresponding dimensions, whose weights are given by the unitary matrix of the gate. 
\Cref{fig:qcs_to_dnn_transformation} demonstrates a transformation from a 3-qubit quantum circuit simulation to DNN computation on a 2$\times$2$\times$2 input tensor. Each element of the input (output) tensor corresponds to a state of the original (new) state vector.

%\ZJ{Comment out the following paragraph as quantum circuit simulation is generally considered memory bound instead of compute bound.}
%DNNs, like quantum simulation, are computationally intensive to train due to the large training datasets and tensor computations.
%
%Similarly, a quantum circuit simulation is computationally intensive because it manipulates a large state vector by applying gates to one or multiple qubits, which amounts to multiplying a matrix with the state vector.
% In DNNs, we deal with this computational demand by exploiting parallelism, typically by using accelerators such as GPUs.

\Cref{fig:overall} shows an overview of \Sys, which uses the aggregated DRAM across multiple nodes to save the state vector of a quantum circuit.
To distribute quantum circuit simulation across multiple GPUs, \Sys divides an input circuit into multiple stages and performs qubit remapping between stages to dynamically adjust how {\em logical} qubits of a quantum circuit map to {\em physical} qubits supported by \Syss underlying simulation system\footnote{In some of the quantum architecture literature, physical qubits refer to the hardware quantum bits.}.
To avoid inter-device communications within each stage, \Sys requires the non-insular qubits of all gates (see \Cref{def:insular_qubit}) to map to local physical qubits (defined in \Cref{def:logical_regional_global} and highlighted by the green lines in \Cref{fig:overall}).

As described in \Cref{sec:background}, simulating the application of a gate to a quantum system requires updating the entire state vector, therefore the simulation of a stage can be considered as the tensor product of the state vector and all gates of the stage. 
%\Sys uses data parallelism to parallelize quantum circuit simulation.
To parallelize a stage's simulation across GPUs, \Sys divides the quantum gates of a stage into kernels, partitions the state vector into multiple batches, and uses data parallelism to process different batches across multiple GPUs in parallel, as shown at the bottom of \Cref{fig:overall}.
%In addition, \Sys divides the quantum gates of a stage into kernels and opportunistically parallelizes the execution of different kernels using pipeline parallelism.
%%%
%\Sys selects the best combination of data and pipeline parallelism for simulating each stage, as shown at the bottom of \Cref{fig:overall}
Achieving efficient quantum circuit simulation on an ML system requires addressing two key challenges.

\subsection{Challenge 1: Inter-Device Communications}
We can simulate a quantum gate by performing a matrix
multiplication, where the stride of memory accesses depends on the
position of the qubit that the gate operates on (\Cref{eqn2}).
%
For example, applying a 1-qubit gate to the $q$-th qubit of a quantum
system involves accessing two states separated by $2^q$ other states.
%
When $2^q$ exceeds the batch size, the accesses will be in different
batches and result in fine-grained inter-device or inter-node
communications.

%%%
Existing ML systems do not easily support these fine-grained communications.
TensorFlow~\cite{Tensorflow} and PyTorch~\cite{pytorch} leverage independence between training samples and use data parallelism to partition samples into multiple batches, which are processed by GPUs in parallel. Data parallelism avoids inter-device communications during the forward processing and backward propagation of a training iteration and only requires communications between iterations.
%This DNN parallelization strategy avoids inter-device communications within a pipeline stage and only requires communications between consecutive stages.

%and/or pipeline parallelism by partitioning input samples or the DNN models across multiple devices, while samples are independent and do not require inter-sample dependencies.

%By leveraging data and pipeline parallelism, existing deep learning systems only need to handle coarse-grained inter-node communications without inter-sample dependencies. Specifically, data parallelism does not require any communications in the forward processing and backward propagation phases, and inter-node communications are only performed to synchronization gradients across devices using AllReduce. In pipeline parallelism, DNN models are partitioned into disjoint stages and communications are not performed between consecutive pipeline stages.

To eliminate fine-grained inter-device communications in quantum circuit simulation and align with the communication pattern of modern DNN systems, \Sys applies {\em qubit remapping} to adjust how {\em logical} qubits in a quantum circuit map to {\em physical} qubits supported by \Sys. Qubit remapping requires all-to-all communications between nodes. To minimize these communications, we formalize qubit remapping as a constrained optimization problem and develop a binary integer linear programming (ILP) algorithm to discover an optimal qubit remapping strategy that minimizes communications.
\Syss {\em circuit partitioner} uses the qubit remapping strategy discovered by the ILP algorithm to split an input circuit into disjoint subcircuits, each of which is assigned to a stage, as shown in \Cref{fig:overall}.


\subsection{Challenge 2: Low Arithmetic Intensity}
Because quantum gates typically operate on a small number of qubits,
simulating a quantum gate typically involves multiplying a small
matrix with a large portion of the state vector.
%
This in turn results in low arithmetic intensity, e.g., as little as  
0.5~\cite{haner_05_2017} for simulating real-world quantum circuits.
%
ML systems use {\em operator fusion} to increase the arithmetic
intensity of DNN computation while reducing GPU memory accesses and
kernel launch overheads.
%
Similarly, in \Sys we execute a subcircuit in a single CUDA kernel by
performing {\em circuit kernelization}.

ML systems perform operator fusion by considering locally connected
DNN operators (e.g., a convolution followed by a ReLU activation) and
applying graph transformations to merge operators~\cite{jia2019taso,
  wang2021pet}.
%
In quantum simulation, we can kernelize any convex, possibly
disconnected, subcircuit. For example, the two gates assigned to
kernel $K_5$ are disconnected in \Cref{fig:overall}.
%
We, therefore, have more advanced optimization opportunities for
kernelizing a circuit and applying existing local-transformation-based
operator fusion techniques will miss opportunities to increase
arithmetic intensity.
%%%
We formalize circuit kernelization as an optimization problem and
propose a novel dynamic programming algorithm to partition the gates
within a stage into kernels while minimizing the aggregated execution
time of these kernels.

We describe \Syss ILP-based circuit partitioner in \Cref{sec:partitioner} and DP-based circuit kernelizer in \Cref{sec:kernelizer}.

\begin{figure*}
    \centering
    \includegraphics[scale=0.36]{figures/overview.pdf}
    %\vspace{-2em}
    \caption{An overview of \Sys. \Syss circuit partitioner splits an input circuit into multiple stages and updates qubit mapping between stages so that the non-insular qubits of each gate (see \Cref{def:insular_qubit}) map to local physical qubits (i.e., green lines in each stage). $q_i[p_j]$ indicates the $i$-th logical qubit maps to the $j$-th physical qubit. \Syss circuit kernelizer further partitions the gates of each stage into kernels, which are executed using data parallelism.}
    \label{fig:overall}
\end{figure*}


==> design.tex <==
%\section{System Design}




==> discussion.tex <==
\section{Limitations and Discussion}
\paragraph{\Syss optimality.} \Syss circuit partitioner uses a 0-1 integer linear programming algorithm to discuss a qubit remapping strategy that minimizes the number of inter-node qubit remappings. \ZJ{Discuss \Sys hierarchical qubit remapping strategy.}
For each partitioned quantum subcircuit, \Syss gate execution scheduler uses a dynamic programming algorithm to fuse gates into DNN kernels while minimizing kernel execution time on GPUs. While both algorithms can discover optimal strategies at their respective level of the optimization stack, \Sys does not guarantee that the end-to-end execution plan discovered by the two algorithms is globally optimal, since a suboptimal circuit partitioning strategy may enable additional optimizations for fusing gates into DNN kernels. However, the combination of these algorithms has demonstrated strong emperical performance for a variety of quantum applications.


==> dp_old.tex <==
\section{Circuit Kernelizer}
\label{sec:kernelizer}
%\section{Gate Fusion Optimizer}

After partitioning an input circuit into multiple stages, \Sys must
efficiently execute the gates of each stage on GPUs.
%
Computations on GPUs are organized as {\em kernels}, each of which is
a function simultaneously executed by multiple hardware threads in a
single-program-multiple-data (SPMD) fashion~\cite{darema1988spmd}.
%
A straightforward approach to executing gates is launching a kernel
for each gate, which yields suboptimal performance due to low arithmetic intensity of each gate.

To improve simulation performance on GPUs, \Sys kernelizes each
stage by partitioning the gates of a stage into kernels.
%
We formulate circuit kernelization as an optimization problem (introduced below) and propose a novel dynamic programming algorithm to solve it. 
%

In \Sys, each {\em kernel} consists of a number of gates. For a
given quantum circuit $\m{C} = (\m{G}, \m{E})$, a kernel is a set of
gate $\m{K} \subseteq \m{G}$ that forms a convex subgraph of
$\m{G}$.
%
A kernel $\m{K}$ forms a convex subgraph of $\m{C} = (\m{G}, \m{E})$,
if for any two gates $g_1, g_2 \in \m{G}'$, all paths in $\m{C}$ from
$g_1$ to $g_2$ are in $\m{K}$.
%
We define the qubits of a kernel $\m{K}$ as the union of the qubits of
the gates in $\m{K}$.


Given a kernel $\m{K}$ in a circuit, \Sys considers two different ways of
executing it.
%
The first way is to compute the unitary matrix of the kernel and execute the kernel via matrix multiplication.
%
For a kernel with $q$ qubits, the unitary matrix is a $2^q \times 2^q$
complex matrix and therefore, the cost of matrix multiplication is
proportional to $O(2^q)$ per element in the state vector.
%
The second approach applies the quantum gates of a kernel by
leveraging the {\em shared memory} available on modern GPUs.
%
When executing a kernel in shared memory, we load the state vector into
the shared memory in batch and apply the gates in the kernel to each
minibatch.
%
To ensure that the kernel always remains in the shared memory, we
bound its size by the size of the GPU's shared memory.
%
In this approach, the cost of executing a kernel is proportional to
the number of gates, plus a constant per element in the state vector
(needed for the transfer of the state vector between the shared memory and
the main memory of a GPU).


%% \subsection{Dynamic Programming for Gate Fusion}
%% \label{subsec:dp}

\begin{problem}[Optimal circuit kernelization]

Given a cost function $\Call{Cost}{\cdot}$ that maps a kernel to its cost (i.e., a real number),
%
the optimal circuit kernelization problem takes as input
%
a quantum circuit $\m{C}=(\m{G}, \m{E})$
%
and
%
returns a feasible schedule of kernels $\m{K}_0,...,\m{K}_{b-1}$ (\,$\not\exists i < j$ such that $\m{K}_i$ depends on $\m{K}_j$) that minimizes
the total execution cost:
\begin{equation}
\sum_{i=0}^{b-1} \Call{Cost}{\m{K}_i}
\label{eqn:dp_objective}
\end{equation}
subject to 
\begin{equation}
\bigcup_{i=0}^{b-1} \m{K}_i = \m{G} ~\mbox{and}~ \m{K}_i \cap \m{K}_j = \emptyset ~\mbox{for}~ i \neq j.
\end{equation}
\label{problem:kernelization}
\end{problem}


\begin{figure}
    \centering
    \subfloat[Sequence\\representation]{
    \includegraphics[scale=0.5]{figures/sequence.pdf}
    \label{fig:sequence}
    }
    \subfloat[An example state of \Sys's dynamic programming.]{
    \includegraphics[scale=0.5]{figures/dp_state.pdf}
    \label{fig:dp_state}
    }
    \vspace{-1em}
    \caption{\Cref{fig:sequence} shows a sequence representation for the quantum circuit in \Cref{fig:dp_state}.}
    \label{fig:my_label}
\end{figure}


%\UA{The description of the DP algorithm is informal.  We need to do
% more work to get this right, but we do not have time before the
% deadline.  So we are avoiding definitionts, etc.}

%% \paragraph{DP state.}
%% \Sys uses a dynamic programming (DP) algorithm to decide how to fuse gates into kernels and how to execute each kernel (e.g., linear or shared-memory kernels).

Note that the above problem definition assumes all kernels are executed sequentially on GPUs (i.e., the summation term in \Cref{eqn:dp_objective}. This is because each kernel updates the entire state vector and therefore cannot be executed in parallel with others.

We present a dynamic programming (DP) algorithm that solves the
optimal circuit kernelization problem.
%
The algorithm maintains a set of kernels along with a set of
\defn{extensible qubits} for each kernel. 
Extensible qubits are qubits that can be connected to another
gate without breaking the convexity of the kernel and without creating cyclic dependencies between kernels. 
%
The DP algorithm represents a circuit as a sequence of gates that
matches a topological sort of gates in the circuit.
%
For example, \Cref{fig:sequence} shows a valid sequence representation for the quantum circuit in \Cref{fig:dp_state}.
%

Given a circuit represented as a sequence of gates, the DP algorithm,
shown in \Cref{alg:dp}, starts by initializing the DP state, and adding the gates of the circuit one by one in
the increasing order.
% 
The DP state is indexed by a position $i$ (starting from zero) and a
kernel set $\KS{}$ at that position; it maps the position and the kernel
set to a cost (a real number) and a set of \defn{closed kernels} up to that position. Closed kernels are kernels with no extensible qubits, so we cannot add any gates to them.
The DP state represents the best kernelization solution containing the kernel set $\KS{}$ up to position $i$: the closed kernels represent the best kernelization of the first $i$ gates excluding $\KS{}$, and the cost of the DP state is the total cost of closed kernels.
%


\Cref{fig:dp_state} shows an example DP state $(i, \KS{})$ with $i = 7$ and $\KS{} = \{\m{K}_1, \m{K}_2\}$. 
Note that the extensible qubit set for $\m{K}_1$ only includes $q_3$, since we can only add future gates operating on $q_3$ (e.g., $g_8$) into $\m{K}_1$. Adding a gate operating on other qubits (e.g., $g_7$ on $q_1$ and $q_2$) into $\m{K}_1$ violates the convexity of the kernel $\m{K}_1$. 
Note that $\KS{}$ does not include kernels with no extensible qubits (e.g., the kernel for $g_0$ and $g_1$ is not in $\KS{}$), this is because we cannot add any future gates into a kernel with no extensible qubits. This simplification helps us reduce the complexity of the DP algorithm.


% To add a gate to the DP state, the algorithm considers each kernel
% state set $\KS{}$ and updates the kernels and their state by
% considering the impact of the gate to each kernel.
% %
% Specifically, there are three cases.  
% %
% In the first case, the gate lies an non-extensible qubit and therefore
% the kernel remains unaffected by this gate.
% %
% In the second case, ...
% %
% In the third case, ..

To add the $i$-th gate $\m{C}[i]$, the algorithm considers each DP state $(i,\KS{})$ and updates the DP state by considering the
impact of the gate on each kernel.
%
When adding a gate, there are two possibilities:
%
The first is to create a singleton kernel consisting of the gate
(Lines~\ref{dp:new_kernel_begin}--\ref{dp:new_kernel_end} in
\Cref{alg:dp}).
%
The second is to add the gate to an existing kernel, if all input
qubits of the gate are extensible
(Lines~\ref{dp:existing_kernel_begin}--\ref{dp:existing_kernel_end} in
\Cref{alg:dp}).
%
In either case, we check if any kernel's extensible qubit set becomes empty after adding the gate, \emph{close} such kernels, and record their costs.
% In each case, we update the extensible qubit set for each kernel state
% after adding the gate by checking if there will be no feasible
% schedules for all kernels in $\KS{}$ if we append a single-qubit gate
% for each qubit (line~\ref{dp:feasible_schedule}); more details on this
% will be described in \Cref{subsec:dp_optimizations}.  We then
% \emph{close} the kernels with empty extensible qubit sets
% (line~\ref{dp:close_begin} to line~\ref{dp:close_end}) and record
% their cost (line~\ref{dp:record_cost}).


% \MX{This is the definition, not property}
% \begin{theorem}
% For a circuit with sequence representation $L=(g_0,g_1,...,g_{m-1})$ and a kernel state \KS{} with fused gates $\m{G}'$ and extensible qubits $\m{X}'$ at the $(i-1)$-th iteration, we can fuse $g_i$ into the kernel if and only if $g_i$'s qubits are a subset of $\m{X}'$.
% \end{theorem}


\begin{figure*}
\begin{minipage}{\textwidth}
%\begin{algorithm}
{
% MX: comment out \small if we have space
\small
\begin{algorithmic}[1]
\Function{$\Call{Kernelize}{}$}{$\m{C}$}

\State {\bf Input:} A quantum circuit $\m{C}$ represented as a sequence of gates.
\State {\bf Output:} A set of kernels.
\State //  $DP[i,\KS{}]$ maps position $i$ and the kernel set $\KS{}$ at that position to the lowest cost and the corresponding closed kernels.

\State $DP[0,\emptyset] = (0, \emptyset)$
% \State $Q = \bigcup_{gate \in \m{C}} {qubits(gate)}$
\For {$i = 0$ \textbf{to} $\Call{Length}{\m{C}}-1$} \label{dp:loop_i}
\For {\textbf{each} $DP[i,\KS{}]$} \label{dp:loop_ks}
\State {\em // Create a new singleton kernel for the gate $\m{C}[i]$.} \label{dp:new_kernel_begin}
\State $c, \KS{}' = \Call{CloseKernels}{\KS{} \cup \{\{\m{C}[i]\}\}}$ \label{dp:new_kernel_close_kernel}
\State $DP[i+1, \KS{}'] = \min(DP[i+1, \KS{}'], DP[i,\KS{}] + c)$ \label{dp:new_kernel_end}
\State {\em // Try to add the gate $\m{C}[i]$ to an existing kernel.} \label{dp:existing_kernel_begin}
\For {$\m{K} \in \KS{}$} \label{dp:loop_k}
\If {$qubits(\m{C}[i]) \subseteq \Call{ExtensibleQubits}{\m{K},\KS{}}$} \label{dp:check_gate}
\State $c, \KS{}' = \Call{CloseKernels}{\KS{} \setminus \{K\} \cup \{\m{K} \cup \{\m{C}[i]\}\}}$ \label{dp:existing_kernel_close_kernel}
\State $DP[i+1, \KS{}'] = \min(DP[i+1, \KS{}'], DP[i,\KS{}] + c)$\label{dp:existing_kernel_end}
\EndIf
\EndFor
\EndFor
\EndFor
\State $ DP_{best} = \min_{\KS{}}\left\{f[\Call{Length}{\m{C}},\KS{}]+\left(\sum_{\m{K}\in\KS{}}\Call{Cost}{\m{K}}, \KS{}\right)\right\}$ \label{dp:compute_f_best}
%\State {\em // $DP_{best}$ is of the form $(DP_{best}.cost, DP_{best}.kernels)$.}
\State \Return $DP_{best}.kernels$
\EndFunction

\State
%\State {\em // Block the gate's qubits from all kernel states in $\KS{}$, return the closed kernels and the remaining kernel states.}
\State // Close the kernels with no extensible qubits in $\KS{}$, return the closed kernels with their cost and the remaining kernels.
\Function{$\Call{CloseKernels}{}$}{$\KS{}$}
\State $closed = \{\m{K} \in \KS{} \mid \Call{ExtensibleQubits}{\m{K},\KS{}} = \phi\}$
\State $\KS{}' = \KS{} \setminus closed$
% \For {$K \in \KS{}$}
% \For {$q \in xqubits(K)$}
% \If {there will be no feasible schedules for all kernels in $\KS{}$ if we append a single-qubit gate on $q$ to $K$} \label{dp:feasible_schedule}
% \State $xqubits(K) = xqubits(K) \setminus \{q\}$
% \EndIf
% \EndFor
% \If {$\Call{ExtensibleQubits}{K,\KS{}} = \emptyset$} \label{dp:close_begin}
% \State $closed \leftarrow closed \cup \{kernel(K)\}$
% \State $\KS{} \leftarrow \KS{} \setminus \{K\}$ \label{dp:close_end}
% \EndIf
% \EndFor
% \State $unaffected = \{K \in \KS{} \mid \forall g \in kernel(K), qubits(g) \cap qubits(gate) = \emptyset; qubits(gate) \subseteq xqubits(K)\}$ \label{dp:unaffected}
% \State $blocked = \{(kernel(K), xqubits(K) \setminus qubits(\m{C}[i])) \mid K \in \KS{} \setminus unaffected\}$ \label{dp:blocked}
% \State $closed = \{kernel(K) \mid K \in blocked; xqubits(K) = \emptyset\}$ \label{dp:closed}
% \State $\KS{}' = \{K \mid K \in blocked; xqubits(K) \neq \emptyset\} \cup unaffected$
\State \Return $\left(\left(\sum_{kernel \in closed}\Call{Cost}{kernel}, closed\right), \KS{}'\right)$ \label{dp:record_cost}
\EndFunction
\end{algorithmic}
}
%\end{algorithm}
\end{minipage}
\vspace{-1em}
\caption{The dynamic programming algorithm. %$xqubits$ means the extensible qubit set of a kernel state.
The ``+'' operator between $(cost, kernels)$ (the value of $DP[i,\KS{}]$) means adding the cost and taking the union of the $kernels$ set.}
\label{alg:dp}
\end{figure*}

\begin{theorem} [Optimality of \Sys's DP algorithm]
The dynamic programming algorithm in \Cref{alg:dp} can discover a list of kernels that minimizes the total execution cost defined in \Cref{eqn:dp_objective}.
\end{theorem}
\begin{proof}
Suppose the feasible schedule of kernels that minimizes the total execution cost defined in \Cref{eqn:dp_objective} is $\m{K}'_0, \m{K}'_1, \dots, \m{K}'_{b'-1}$. For each kernel $\m{K}'_j$, its gates can be ordered as a subsequence in $\m{C}$. We denote the intersection of a kernel $\m{K}'_j$ and a prefix of gates $\m{C}[0\dots i-1]$ as $\m{K}'_j[\m{C}(i)]$.

We prove by induction on $i$ that there is a DP state $(i,\KS{})$ before the iteration $i$ of the loop in Line~\ref{dp:loop_i} in \Cref{alg:dp} (or before Line~\ref{dp:compute_f_best} if $i=\Call{Length}{\m{C}}$) such that 
\begin{align}
&\forall \m{K}'_j \neq \m{K}'_j[\m{C}(i)] \neq \emptyset, \m{K}'_j[\m{C}(i)] \in \KS{} \label{eqn:ind_hyp} \\
&\forall \m{K}'_j = \m{K}'_j[\m{C}(i)], \m{K}'_j \in \KS{} \cup DP[i,\KS{}].kernels\label{eqn:ind_hyp2}
\end{align}
for $0 \le i \le \Call{Length}{\m{C}}$. These hold for $i=0$ because $\m{K}'_j[\m{C}(0)] = \emptyset$ for all $j$.

Suppose \cref{eqn:ind_hyp,eqn:ind_hyp2} hold for $i < \Call{Length}{\m{C}}$, and we prove that they hold for $i+1$. 
We pick $j$ such that the gate $\m{C}[i]$ is in $\m{K}'_j$. Suppose we are executing the iteration of $\KS{}$ satisfying \cref{eqn:ind_hyp,eqn:ind_hyp2} for $i$ of the loop at Line~\ref{dp:loop_ks} in \Cref{alg:dp}. Applying \cref{eqn:ind_hyp} on $i$ and $j$, we get two cases:
\begin{enumerate}
\item $\m{K}'_j[\m{C}(i)] = \emptyset$, then $\m{K}'_j[\m{C}(i+1)] \in \KS{}'$ holds before calling $\Call{CloseKernels}{}$ at Line~\ref{dp:new_kernel_close_kernel};
\item $\m{K}'_j[\m{C}(i)] \in \KS{}$, then we must have $qubits(\m{C}[i]) \subseteq \Call{ExtensibleQubits}{\m{K},\KS{}}$ because adding $\m{C}[i]$ to this kernel results in a feasible schedule that is a sub-sequence of $\m{K}'_0[\m{C}(i)],\m{K}'_1[\m{C}(i)],\dots, \m{K}'_{b'-1}[\m{C}(i)]$. When running the iteration $\m{K}'_j[\m{C}(i)]$ of the loop at Line~\ref{dp:loop_k}, $\m{K}'_j[\m{C}(i+1)] \in \KS{}'$ holds before calling $\Call{CloseKernels}{}$ at Line~\ref{dp:existing_kernel_close_kernel}.
%because there is always a feasible schedule that is a subsequence of $\m{K}'_0[\m{C}(i)],\m{K}'_1[\m{C}(i)],\dots, \m{K}'_{b'-1}[\m{C}(i)]$. So \cref{eqn:ind_hyp} holds for $i+1$ after Line~\ref{dp:existing_kernel_end}.
\end{enumerate}
In either case, when calling $\Call{CloseKernels}{}$, the extensible qubit set cannot be empty for any $\m{K}'_{\hat{j}}[\m{C}(i+1)] \neq \m{K}'_{\hat{j}}$ after adding the gate $\m{C}[i]$ because we can put the next gate in $\m{K}'_{\hat{j}}$ into $\m{K}'_{\hat{j}}[\m{C}(i+1)]$. For any $\m{K}'_{\hat{j}}[\m{C}(i+1)] = \m{K}'_{\hat{j}}$, it is possible to move it from $\KS{}$ to $DP[i+1,\KS{}].kernels$. Combining with \cref{eqn:ind_hyp,eqn:ind_hyp2} for $i$, we prove \cref{eqn:ind_hyp,eqn:ind_hyp2} for $i+1$.

Applying \cref{eqn:ind_hyp2} on $i=\Call{Length}{\m{C}}$, we conclude that the optimal schedule is selected in Line~\ref{dp:compute_f_best} and returned.
\end{proof}

\subsection{Optimizations to the DP Algorithm}
\label{subsec:dp_optimizations}
The DP algorithm presented in \Cref{alg:dp} can discover an optimal strategy to kernelize a circuit but is prohibitively expensive to run in practice. This section describes a list of optimizations in \Sys to accelerate the DP algorithm.

\paragraph{Extensible and fixed kernels.}
Tracking the set of extensible qubits for each kernel is expensive. 
One way to simplify the computation of extensible qubits is to maintain a total order for all kernels in $\KS{}$; however, doing so will result in significantly more DP states since different orders of the same set of kernels will be in different DP states. 
Thus, \Sys categorizes kernels into \defn{extensible} and \defn{fixed} kernels, and maintains an order for {\em fixed} kernels in the DP state. 

\begin{definition}[Extensible and fixed kernels]
A kernel $\m{K}$ is extensible if its extensible qubit set is all qubits; otherwise, it is fixed.
\end{definition}

\Cref{fig:dp_with_optimization} shows an example DP state with extensible and fixed kernels. \Sys requires that all extensible kernels are scheduled after fixed kernels (explained later), therefore $\KS{}$ must begin with $\m{K}_2, \m{K}_3$.
By definition, extensible kernels (e.g., $\m{K}_1$ and $\m{K}_4$) do not have any dependencies between each other, which allows them to be scheduled in an arbitrary order after all fixed kernels.

This order for fixed kernels makes it easy to compute the extensible qubit set for each kernel: whenever we add a gate $g$ to a kernel $\m{K}$, we simply remove $g$'s qubits from all extensible qubit sets of kernels before $\m{K}$ in $\KS{}$. 
For the example DP state in \Cref{fig:dp_with_optimization}, (1) adding $g_8$ to an extensible kernel (e.g., $\m{K}_1$ or $\m{K}_4$) will remove $q_2$ and $q_3$ from the extensible qubit sets of all fixed kernels (i.e., $\m{K}_2$ and $\m{K}_3$), (2) adding $g_8$ to $\m{K}_3$ will remove $q_2$ and $q_3$ from the extensible qubit set of $\m{K}_2$, and (3) adding $g_8$ to $\m{K}_2$ does not require updating the extensible qubit set for any kernels since $\m{K}_2$ is the first fixed kernel.
%%%
To avoid introducing cyclic dependencies, we refrain from changing the qubit set of any fixed kernels (another reason why these kernels are fixed).

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/dp_state_with_optimization.pdf}
    \caption{An example DP state in \Sys's implementation.}
    \label{fig:dp_with_optimization}
\end{figure}


\if 0
\ZJ{To be removed <===============}
Checking if we can add a gate to a kernel on the fly (Line~\ref{dp:check_gate} in \Cref{alg:dp}) is expensive, and maintaining the extensible qubit set for each kernel is also expensive. If we maintain an order of the kernels, maintaining the extensible qubit set will only take linear time on the number of qubits for each kernel.
However, maintaining a strict order of kernels in $\KS{}$ would greatly restrain the representability of the DP state; therefore, we compromise by categorizing the kernels into \defn{extensible kernels} and \defn{fixed kernels}.

\begin{definition}[Extensible and fixed kernels]
A kernel $\m{K}$ is extensible if its extensible qubit set is all qubits; otherwise, it is fixed.
\end{definition}

Extensible kernels do not have any dependency on each other. They can be placed arbitrarily in an order of kernels in $\KS{}$ as long as all extensible kernels are placed at the end.

As long as newly added gates do not change any qubit set of kernels of fixed kernels (therefore not creating any new dependencies -- this is why it is called \emph{fixed}), we are able to maintain an order of the kernels in $\KS{}$ where all extensible kernels are placed at the end.

After the order is determined, it will be easy to maintain the extensible qubit set for each kernel: whenever we add a gate to a kernel $\m{K}$, simply remove the gate's qubits from all extensible qubit sets of kernels before $\m{K}$.

\ZJ{=========>}
\fi

\paragraph{Simplifying DP state representation.}
Recall that the DP state described in \Cref{alg:dp} maintains the set of gates for each kernel. However, in a quantum circuit, the number of gates is typically orders of magnitude more than the number of qubits, making it prohibitive to directly track a gate set for each kernel.
To simplify the DP state, \Sys leverages the fact that the cost of a \defn{fusion} kernel (i.e., multiplying the unitary matrix of the kernel) only depends on the number of qubits in the kernel, and the cost of a \defn{shared-memory} kernel $\m{K}$ can be approximated as $\alpha + \sum_{g\in \m{K}} \er{Cost}(g)$, where $\alpha$ is a constant that corresponds to the time to load a micro-batch of state coefficients to GPU shared memory, and $\er{Cost}(g)$ is the cost to simulate the application of the gate $g$ in the GPU shared memory.
Therefore, instead of tracking a gate set for each kernel, \Sys maintains the set of qubits the kernel operates on for extensible kernels or its intersection with the extensible qubit set for fixed kernels.
For example, we only need to keep track of the set $\{q_4,q_5\}$ for the fixed kernel $\m{K}_2$ in \Cref{fig:dp_with_optimization} because we can only add gates operating only on these qubits to $\m{K}_2$.
This approach significantly simplifies the representation of a DP state and reduces the number of DP states \Sys considers.

\paragraph{\Kwins{} qubits.}
Recall that \Sys's circuit partitioner allows mapping the insular qubits of a gate to regional and global qubits. 
Before loading a batch of states to GPU, the values of all global and regional qubits for the batch are known, which are leveraged by \Sys to simplify computation.
Specifically, for gates with \kwins{} non-local qubits, \Sys retrieves the non-local qubits' values and converts these gates into local gates with fewer qubits.

This optimization is also applicable to shared-memory kernels. A physical qubit is \defn{active} for a shared-memory kernel if its states are loaded into the shared memory in a single micro-batch. 
For \emph{non-active} local qubits, \Sys applies a similar optimization to gates with \kwins{} non-active local qubits that converts these gates into smaller gates with only active qubits.
%%%
In order to know when a shared-memory kernel $\m{K}$ is no longer extensible, \Sys tracks the non-active qubit set for $\m{K}$ when $\m{K}$ is extensible. 
When converting $\m{K}$ to a fixed one, \Sys computes $\m{K}$'s extensible qubit set to place \kwins{} qubits of future gates.

% \ZJ{This seems like implementation details. I would suggest we remove this paragraph.} \Sys also attaches a gate if it has exactly one local qubit. 
% If there is no other gate on the local qubit in this stage, we first try to attach the gate to a gate in the next stage if this gate still has exactly one local qubit in the next stage, and simply keep the gate if it cannot find a good place to attach.


%on each qubit is a common pattern at the beginning of some circuits. They cause an exponential blowup in the number of different DP states.
%Note that there should not be any qubit with only single-qubit gates (otherwise the qubit is not entangled in the circuit), we attach each single-qubit gate to an adjacent multi-qubit gate.

%If a single-qubit gate's qubit is non-\kwins{}, we need to mark the corresponding qubit in the multi-qubit gate it attaches to as non-\kwins{}.

%If both the single-qubit gate's qubit and the corresponding qubit in the adjacent multi-qubit gate are \kwins{} (the corresponding qubit in the multi-qubit gate should be a control qubit here), we can swap these two gates instead of attaching without affecting the execution result, making the single-qubit gate possible to be merged with some other single-qubit gates on the same qubit. Note that as shown in \Cref{fig:swap}, if the single-qubit gate's matrix is anti-diagonal (e.g., the $X$ gate), we need to flip the control state of the corresponding control qubit of the multi-qubit gate -- if the control state was $\ket{1}$, we need to flip it to $\ket{0}$ after swapping.


%\ZJ{@mingkuan: I rewrote this paragraph and dropped some details. Take a look and let me know if you think some details are important and must be mentioned here.}

\if 0
\MX{The following is wrong and misses important details. Fixed fusion kernels and fixed shared-memory kernels are very different. We need to keep track of one set which is the intersection of the kernel's qubits and the extensible qubit set for both kernels, but we need to keep track of an additional set which is the extensible qubit set for shared-memory kernels. This is also why I put "Insular qubits and shared-memory kernels" before this paragraph -- that optimization affects this which causes significant changes in the index of DP states. So I don't think we can leave that in the implementation details.}
\ZJ{I see. I moved the insular qubit part back to this section.}
%Therefore, instead of tracking a gate set for each kernel, \Sys maintains the kernel type (i.e., fixed or extensible) and its set of qubits. For each fixed kernel, \Sys also tracks its set of extensible qubits, which is a subset of its qubit set. 
%This approach significantly reduces the number of DP states \Sys considers.

\ZJ{Old version <=========}
\paragraph{Maintaining the minimum necessary for the cost function}
Recall that $\Call{Cost}{\cdot}$ maps a kernel to its cost, which requires keeping all the gates in a kernel. However, the number of gates can be much more than the number of qubits, and keeping them may cause the DP state to be too large.

In our implementation, the cost of a \defn{fusion kernel} (computing the unitary matrix representation of the kernel) is only related to the number of qubits in the kernel, and the cost of a \emph{shared-memory kernel} is a constant number for the initialization cost plus a cost for each gate (which can vary for different types of gates). Therefore, we keep track of the type for each kernel at the beginning, and we only need to keep track of the qubit set (which is also necessary to the DP itself). Whenever we add a gate to a shared-memory kernel, we record the cost of the gate immediately instead of when recording the cost of the kernel.

We do not keep track of extensible qubit sets for extensible kernels because they are defined to be all qubits. When we generate a fixed kernel, we need to keep track of its extensible qubit set; but recalling that newly added gates cannot change any qubit set of kernels of fixed kernels, we only need to keep track of the intersection of the extensible qubit set and the qubit set of the kernel, which is much smaller and is essentially the qubit set excluding the qubits in the gate which caused the generation of the fixed kernel. For a fixed shared-memory kernel, however, we still need to compute its extensible qubit set: we need to keep track of this set in order to place \kwins{} qubits.

We record the cost of a kernel when generating the fixed kernel because its cost will not change anymore for fusion kernels and its initialization cost will not change anymore for shared-memory kernels. We simply remove a fixed kernel when its qubit set becomes empty.
\ZJ{=========>}
\fi 

\paragraph{Optimizing DP transition.}
When a new gate $g$ can be subsumed by an existing kernel $\m{K}$ or vice versa (this happens when $\m{K}$ is an extensible kernel and $\m{K}$'s qubits are a subset of $g$'s),
\Sys directly adds $g$ into $\m{K}$.
For example, in \Cref{fig:dp_with_optimization}, \Sys will directly add $g_7$ into $\m{K}_4$ without considering other options.
This optimization greatly reduces the amount of DP transitions \Sys must explore.

\paragraph{Deferring adding gates to extensible kernels.}
To further reduce the number of DP states, we keep gates as single-gate kernels when they are extensible instead of trying to add them to each of the extensible kernels. Whenever we need to convert an extensible kernel to a fixed one, we search for all other extensible kernels to be merged together at that time. For example, after adding $g_7$ into $\m{K}_4$ in \Cref{fig:dp_with_optimization}, we create a singleton kernel $\m{K}_5$ for $g_8$. Since $\m{K}_4$ will become fixed after the creation of $\m{K}_5$, we can merge $\m{K}_4$ with $\m{K}_5$ to form a new extensible kernel (which is equivalent to adding $g_8$ to $\m{K}_4$), or merge $\m{K}_4$ with $\m{K}_1$ to form a fixed kernel (which is equivalent to adding $g_6$ and $g_7$ to $\m{K}_1$ instead of creating $\m{K}_4$ at the beginning). Either way, we do not consider the option of adding $g_8$ to $\m{K}_1$, which will eventually either be considered by merging $\m{K}_5$ with $\m{K}_1$ later or be deemed unnecessary.

%When merging multiple extensible kernels to generate a fixed kernel, \Sys restricts the maximum number of qubits for shared-memory kernels based on the GPU shared memory size and also sets a maximum number of qubits for fusion kernels where the cost will become too high otherwise.

Recall that \Sys tracks the \kwins{} qubits for shared-memory kernels. To defer merging extensible kernels as far as possible, \Sys keeps multiple shared-memory kernels as extensible even if they share \kwins{} qubits. This optimization may require swapping adjacent gates that share a \kwins{} qubit, which will be described in the next paragraph.


%\ZJ{What is merging extensible kernels to generate fixed kernel?}\MX{See the paragraph "Deferring merging kernels".} \ZJ{What's a reasonable cost?} \MX{The cost function for kernels gives us the cost of fusion kernels for each number of qubits. When the number of qubits is too high, the cost can be prohibitive because it is proportional to two to the power of the number of qubits.}

\if 0
\ZJ{Old version <====================}
We have some other minor optimizations during the DP transition to reduce the number of DP states.

If a gate is subsumed by an existing kernel, we directly add the gate to that kernel without considering other choices.

If an existing extensible kernel is subsumed by a new gate (this may happen if the existing kernel consists of one gate and the new gate operates on all qubits in the existing gate and also some other qubits), we add the new gate to that kernel without considering other choices.

When merging extensible kernels to generate fixed kernels, we restrict the maximum size for shared-memory kernels, and also set a maximum size for fusion kernels based on a reasonable cost.

\ZJ{====================>}
\fi

\paragraph{Attaching single-qubit gates.}
Our preliminary experiments showed that the single-qubit gates of a quantum circuit could easily result in an exponential blowup in the number of DP states because of the independence between single-qubit gates applied to different qubits. To address this issue, we attach each single-qubit gate to an adjacent multi-qubit gate using the following rules. First, for a \kwnonins{} single-qubit gate, \Sys merges the gate into an adjacent multi-qubit gate and marks the corresponding qubit \kwnonins{}. Second, in the case where the single-qubit gate $g_1$ is \kwins{} and connects to the control qubit of a multi-qubit gate $g_2$, \Sys swaps these two gates, which allows $g_1$ to be merged with other subsequent single-qubit gates. 
Note that if the unitary matrix of $g_1$ is anti-diagonal (e.g., the $X$ gate), \Sys flips the control state of $g_2$, as shown in \Cref{fig:swap}.

\begin{figure}[tb]
    \centering
    \includegraphics[scale=0.4]{figures/swap_cx0.pdf}
    \vspace{-1em}
    \caption{If we swap an $X$ gate with an adjacent $CX$ gate, we need to flip the control state of the new $CX$ gate to $\ket{0}$.}
    \label{fig:swap}
\end{figure}

\paragraph{Post-processing}
After the DP algorithm, \Sys needs to convert all kernels in $\KS{}$ into closed kernels as a post-processing step, which requires merging kernels. 
Computing the minimum cost for merging kernels is NP-hard because the bin packing problem can be reduced to this problem.
\Sys uses a simple approximation algorithm that greedily packs the kernels in $\KS{}$ into closed kernels, running in quasilinear time: (1) for fusion kernels, \Sys merges them into closed kernels based on their cost-efficient density; (2) for shared-memory kernels, \Sys packs them into closed kernels towards the maximum shared-memory kernel size.

\paragraph{Pruning DP states.}
Another key optimization to reduce the DP states is {\em pruning}. A simple pruning based on the cost of the DP states would be suboptimal because we have not considered the cost of the extensible kernels which may contribute a lot.
%%%
%Because the number of DP states is still too high, we need to prune some of them during the DP. However, we cannot simply take the minimum cost among DP states because we have not considered the cost of the kernels which may contribute a lot.
During the DP, whenever the number of states at the same position $i$ in the circuit reaches a user-defined threshold $T$ at the beginning of an iteration (i.e., Line~\ref{dp:loop_i} in \Cref{alg:dp}), \Sys performs the post-processing step introduced above at the current position for all DP states and keeps $\frac{T}{2}$ DP states with the lowest cost after post-processing.
%we compute the ``kernel schedule at the end'' at the current position for each DP state to get the cost of kernels in $\KS{}$, and keep only the 1,000 DP states with the lowest total cost of kernels in $\KS{}$ and closed kernels.
Our preliminary experimentation with this pruning suggested that it does not affect \Sys's results. % \MX{I didn't do any experiment to back up this} \SC{I did it for 28-qft, treid 1000,2000,4000,8000, do we want to report it?}
We set $T = 2,000$ in our evaluation, which achieves good performance.



%% \section*{Old Version}

%% The DP algorithm takes a sequence of gates $L = (g_1,g_2,...,g_k)$ as input and iteratively decides how to add each gate to existing kernels or create a new kernel for the gate. At a given iteration, existing kernels can be categorized into {\em expandable} and {\em fixed} kernels, which are defined as follows.

%% \begin{definition} [Expandable and fixed kernels.]
%% \ZJ{Mingkuan, check whether this definition is correct.}
%% For a given sequence of gates $L = (g_1,g_2,...,g_k)$, a kernel $\m{K}$ is a {\em expandable} kernel there does not exist a gate $g_i \in \m{K}$ and $g_j \notin \m{K}$ such that $g_j$ depends on $g_i$. Otherwise, the kernel $\m{K}$ is a {\em fixed} kernel for sequence $L$.
%% \end{definition}

%% \ZJ{Not sure if we need to define prefix of a sequence here.}
%% Intuitively, a kernel $\m{K}$ is expandable for a sequence of gates if for each of $\m{K}$'s qubit, the sequence does not include any other gates after $\m{K}$, which allows \Sys to potentially fuse $\m{K}$ with subsequent gates while maintaining convexity.
%% %%%
%% On the other hand, a kernel $\m{K}$ is fixed for a sequence of gates if the sequence includes at least one other kernel $\m{K}'$ that depends on $\m{K}$. 
%% This dependency prevents \Sys from fusing arbitrary other gate into $\m{K}$. In this case, \Sys assumes that $\m{K}$'s qubits are {\em fixed} and only considers merging gates operating on $\m{K}$'s qubits into $\m{K}$. 
%% Before merging new gates into $\m{K}$, \Sys also needs to check if the new kernel corresponds to a convex subgraph. 


%% \begin{definition}[Kernel]
%% A kernel is a group of quantum gates to be executed together on GPUs.
%% To be executed together, the gates must form a convex subgraph in the original circuit, i.e., there is no other gate depending on some gate in a kernel and also preceding some gate in the same kernel.

%% For a graph $G$, a subgraph $H$ of $G$ is called \defn{convex} in $G$
%% if for any pair of vertices $u, v$ in $H$, the vertices of every path
%% in $G$ between $u$ and $v$ are contained in $H$.
%% \end{definition}

%% \begin{definition}[Kernel]
%%   A \defn{kernel} in a quantum circuit is a convex subgraph of the
%%   graph for that circuit.
%% \end{definition}

%% Intuitively, a kernel constitutes a subcircuit that can be executed
%% independently as a unit.

%% %% \begin{definition}[Kernel]
%% %% A kernel is a group of quantum gates to be executed together on GPUs.
%% %% To be executed together, the gates must form a convex subgraph in the original circuit, i.e., there is no other gate depending on some gate in a kernel and also preceding some gate in the same kernel. 

%% %% We define the qubits of a kernel to be the union set of the qubits of its gates.
%% %% \end{definition}

%% \begin{definition}[Kernel history]
%% A kernel history is a list of kernels such that executing them sequentially results in a prefix of a stage. \MX{Define stage in sequence representation}
%% \end{definition}
%% \begin{definition}[Open kernel]
%% A kernel in a kernel history is called an open kernel if no later kernels' qubits in the history intersect this kernel's qubits.

%% One important property of open kernels is they can be reordered arbitrarily with other open kernels in a kernel history without changing the execution result.
%% \end{definition}
%% \begin{definition}[Closed kernel]
%% A kernel in a kernel history is called a closed kernel if it is not an open kernel.
%% \end{definition}
%% When doing DP, we cannot put new gates into most closed kernels. But there are exceptions:
%% \begin{definition}[Absorbing kernel]
%% A subset of qubits of a closed kernel's qubits is called an absorbing kernel if no later kernels' qubits in the history intersect this subset.
%% \end{definition}

%% We can then define the DP state to be a set of open kernels and a set of absorbing kernels.

%% Following is the old version.

%% In each stage, we need to execute a sequence of gates. A straightforward way is to launch a CUDA kernel for each gate, but the overhead is high.
%% To reduce the overhead, we can fuse gates in a \emph{convex subgraph} to get a \emph{fusion kernel}. For a fusion kernel, we pre-compute the product of the gate matrices, and launch a kernel with the matrix product.

%% Another way is to utilize GPU's shared memory. A \emph{shared-memory kernel} also consists of a \emph{convex subgraph} of the circuit, but its size is fixed to the size of GPU's shared memory, and the gates are executed one by one instead of being fused to a single matrix. When launching a shared-memory kernel, we load the state vector into the shared memory in batches, and we require the 3 qubits of the least significant bits in the state vector to be always in shared-memory kernels to maximize memory load efficiency (each load consists of at least $2^3 = 8$ complex numbers, or \SI{128}{B}).\MX{Changed from KB to B; also, we should use \textbackslash SI to give the correct space width}

%% \subsection{DP Formulation}

%% We consider the gates in the sequence one by one, adding them to \emph{open kernels}. Open kernels are kernels that can be executed in any order. Whenever there is a dependency, we \emph{close} the kernel that must be executed before some new open kernel. The dynamic programming state (\Cref{alg:dp} line~\ref{dp:state}) maps a prefix of the gate sequence and corresponding open kernels to the minimal total cost of the closed kernels.

%% \begin{figure}[t]
%%     \centering
%%     \includegraphics[scale=0.5]{figures/absorbing_kernel.png}
%%     \caption{After we add the open kernel $O$ and close the kernel $A$, we can still put any gate which only operates on $q_0$ to the \emph{absorbing kernel} $A$.}
%%     \label{fig:absorbing_kernel}
%% \end{figure}

%% However, closing the kernel whenever there is a new gate touching at least one qubit is too conservative. We can put a future gate in the existing closed kernel as long as the future gate only operates on qubits that are in the closed kernel and there are no gates touching any qubit from the point we close the kernel to the location of the future gate, such as the H gate in \Cref{fig:absorbing_kernel}. We call such a closed kernel, excluding any qubit that has been touched by any gate after the kernel is closed, an \emph{absorbing kernel}. An absorbing kernel can absorb any gate that only operates on qubits in it (line~\ref{dp:absorbed}), while it must exclude any touching qubits if any gate operates on it partially (line~\ref{dp:update_absorbing}). We record the set of absorbing kernels, denoted $\m{A}$, in the dynamic programming state (line~\ref{dp:state}).

%% \subsection{Merging Kernels}

%% In order to reduce the number of kernels so as to reduce the overhead of kernel launches, we want to merge some kernels with different qubits. Note that we only merge kernels of the same type (fusion or shared-memory). To reduce the number of dynamic programming states, we delay merging kernels when possible (line~\ref{dp:not_touching}), and only merge them when we are about to close the kernels.

%% When a new gate partially touches some kernels, we assign a new kernel for the new gate, and decide whether to merge each touching kernel with the new kernel (line~\ref{dp:merge_new}) or to close it. If we decide to close the existing kernel, we search for all possibilities to merge it with open kernels (line~\ref{dp:merge_close}), then close it and add it to the set of absorbing kernels.

%% \subsection{End Schedule}
%% In the end, we need to close all open kernels and we may want to merge some of them. Although we do not need to consider any future gates, computing the minimum cost is still NP-hard because the Packing Problem can be reduced to this problem. We use a simple approximation algorithm that greedily packs the open kernels into kernels with the most cost-efficient density for fusion kernels, which is quasilinear to the number of open kernels; for shared-memory kernels, we also greedily pack the open kernels into kernels of the fixed shared-memory kernel size.

%% During the dynamic programming, whenever the number of states grows too high, we can also compute the ``end schedule'' at the current stage for each state to get the cost of open kernels, and prune the states with the total cost of open and closed kernels being too high.

%% \subsection{Removing Single-Qubit Gates}
%% To further reduce the number of states the dynamic programming needs to consider, we have a preprocessing step before the dynamic programming, simply to remove all single-qubit gates. After we get the kernel schedules from the dynamic programming of multi-qubit gates, we insert all the single-qubit gates according to their location in the original circuit sequence into the kernels. If there is no available kernel to insert a gate, we create a single-qubit kernel for it \MX{why is this unlikely?}.



%% % \begin{algorithm}[ht]
%% % \caption{The dynamic programming algorithm.}
%% % \label{alg:dp}
%% % {
%% % %\small
%% % \begin{algorithmic}[1]
%% % \State {\bf Input:} A sequence of quantum gates $seq$ in one stage, the set of local qubits in this stage, and a kernel cost function $\Call{Cost}{\cdot}$.
%% % \State {\bf Output:} A sequence of kernels $schedule$.
%% % \State {\em // $DP[i,\KS{}]$ stores a pair of the minimal cost of the closed kernels and the closed kernels, where the first $i$ gates of $seq$ have been assigned to kernels, and $\KS{}$ is the set of kernel states.} \label{dp:state}
%% % \State $DP[0,\emptyset] = (0, \emptyset)$
%% % \For {$i = 0$ \textbf{to} $\Call{Length}{seq}-1$}
%% % \For {$\KS{}$ such that $DP[i,\KS{}]$ exists}
%% % \State {\em // Try to add the gate to a new kernel.}
%% % \State $c, \KS{}' = \Call{UpdateKernelStates}{\KS{}}$
%% % \State $\KS{}'' = \KS{}' + (seq[i], all\ qubits)$
%% % \State $DP[i+1, \KS{}''] = \min(f[i+1, \KS{}''], f[i,\KS{}] + c)$
%% % \State {\em // Try to add the gate to an existing kernel.}
%% % \For {$KS \in \KS{}$}
%% % \If {$seq[i].qubits \subseteq KS.qubits$}
%% % \State $c, \KS{}' = \Call{UpdateKernelStates}{\KS{} \setminus \{KS\}}$
%% % \State $\KS{}'' = \KS{}' + (KS.gates + seq[i], KS.qubits)$
%% % \State $DP[i+1, \KS{}''] = \min(f[i+1, \KS{}''], f[i,\KS{}] + c)$
%% % \EndIf
%% % \EndFor
%% % \EndFor
%% % \EndFor
%% % \State $\displaystyle f_{best} = \min_{\KS{}}\{f[\Call{Length}{seq},\KS{}]+\left(\sum_{KS\in\KS{}}\Call{Cost}{KS.gates}, \{KS.gates \mid KS \in \KS{}\}\right)\}$
%% % \State {\em // $DP_{best}$ is of the form $(f_{best}.cost, f_{best}.kernels)$.}
%% % \State \Return $DP_{best}.kernels$
%% % \State
%% % \State {\em // Block the gate's qubits from all kernel states in $\KS{}$, return the closed kernels and the remaining kernel states.}
%% % \Function{$\Call{UpdateKernelStates}{}$}{$\KS{},gate$}
%% % \State $blocked = \{KS.qubits \setminus seq[i].qubits \mid KS \in \KS{}\}$
%% % \State $closed = \{KS.gates \mid KS \in blocked, KS.qubits = \emptyset\}$
%% % \State $\KS{}' = \{KS \mid KS \in blocked, KS.qubits \neq \emptyset\}$
%% % \State \Return $\left(\left(\displaystyle\sum_{kernel \in closed}\Call{Cost}{kernel}, closed\right), \KS{}'\right)$
%% % \EndFunction
%% % \end{algorithmic}
%% % }
%% % \end{algorithm}

%% % following is the old version
%% % \begin{algorithm}[ht]
%% % \caption{The dynamic programming algorithm.}
%% % \label{alg:dp}
%% % {
%% % %\small
%% % \begin{algorithmic}[1]
%% % \State {\bf Input:} A sequence of quantum gates $seq$ in one stage, the set of local qubits in this stage, and a kernel cost function $\Call{Cost}{\cdot}$.
%% % \State {\bf Output:} A sequence of kernels $schedule$.
%% % \State {\em // $DP[i][\m{O}][\m{A}]$ stores the minimal cost of the closed kernels (and the closed kernel history) in the schedule where the first $i$ gates of $seq$ are placed in either closed or open kernels, $\m{O}$ stores the collection of open kernels, and $\m{A}$ stores the collection of absorbing closed kernels.} \label{dp:state}
%% % \State $DP[0][\emptyset][\emptyset].cost = 0$
%% % \State $DP[0][\emptyset][\emptyset].kernels = \emptyset$
%% % \For {$i = 0$ \textbf{to} $\Call{Length}{seq}-1$}
%% % %\For {$\m{O}, \m{A}$ such that $DP[i - 1][\m{O}][\m{A}]$ exists}
%% % \For {$\m{O}', \m{A}'$}
%% % \State $DP[i+1][\m{O}'][\m{A}'] = \mathrm{mincost}_{\m{O}, \m{A}}[(\m{O}',\m{A}') \in \{\Call{SearchSpace}{\m{O},\m{A},seq[i]}\}]\{f[i][\m{O}][\m{A}] +$\;newly closed kernel if any$\}$
%% % \EndFor
%% % \EndFor
%% % \State $DP_{best} = \mathrm{mincost}_{\m{O}, \m{A}}\{f[\Call{Length}{seq}][\m{O}][\m{A}]+\Call{Cost}{\m{O}}\}$
%% % \State \Return $DP_{best}.kernels$
%% % \State
%% % \Function{$\Call{SearchSpace}{}$}{$\m{O},\m{A},gate$}
%% % \If {$\exists A \in \m{A}, gate.qubits \subseteq A$} \label{dp:absorbed}
%% % \State \Return $\{(\m{O}, \m{A})\}$
%% % \EndIf
%% % \If {$\exists O \in \m{O}, gate.qubits \subseteq O$} \label{dp:not_touching}
%% % \State \Return $\{(\m{O}, \m{A})\}$
%% % \EndIf
%% % \State $\m{A}' = \{A \setminus gate.qubits \mid A \in \m{A}\}$ \label{dp:update_absorbing}
%% % % \If {$\forall O \in \m{O}, gate.qubits \cap O = \emptyset$}
%% % % \State \Return $\{\m{O} \cup \{gate.qubits\}, \m{A}\}$ % gate.qubits is a set, so \{gate.qubits\} is a set of set
%% % % \EndIf
%% % \State $touching\_kernels = \{O \in \m{O} \mid gate.qubits \cap O \neq \emptyset\}$
%% % \State $\m{O}' = \m{O} \setminus touching\_kernels$
%% % \State \Return $\Call{Search}{touching\_kernels, \m{O}', \m{A}', gate.qubits}$
%% % \EndFunction
%% % \State
%% % \Function{$\Call{Search}{}$}{$touching\_kernels, \m{O}', \m{A}', new\_kernel$}
%% % \If {$touching\_kernels = \emptyset$}
%% % \State \Return $\{(\m{O}' \cup \{new\_kernel\}, \m{A}')\}$
%% % \EndIf
%% % \State Pick any $O \in touching\_kernels$.
%% % \State {\em // Either merge with the new kernel...}
%% % \State $result = \Call{Search}{touching\_kernels \setminus O, \m{O}', \m{A}', new\_kernel \cup O}$ \label{dp:merge_new}
%% % \State {\em // ... or merge with some kernels and close it.}
%% % \For {$merging\_kernels \subseteq \m{O}'$} \label{dp:merge_close}
%% % \State $closed\_kernel = O \cup \left(\bigcup merging\_kernels\right)$
%% % \State $result = result \cup \Call{Search}{touching\_kernels \setminus O, \m{O}' \setminus merging\_kernels, \m{A}' \cup \{closed\_kernel \setminus new\_kernel\}, new\_kernel}$
%% % \EndFor
%% % \State \Return $result$
%% % \EndFunction
%% % \end{algorithmic}
%% % }
%% % \end{algorithm}




==> dp_old2.tex <==
% 2023/11/25
\section{Circuit Kernelizer}
\label{sec:kernelizer}
%\section{Gate Fusion Optimizer}

After partitioning an input circuit into multiple stages, \Sys must
efficiently execute the gates of each stage on GPUs.
%
GPU computations are organized as {\em kernels}, each of which is
a function simultaneously executed by multiple hardware threads in a
single-program-multiple-data (SPMD) fashion~\cite{darema1988spmd}.
%
A straightforward approach to executing gates is launching a kernel
for each gate, which yields suboptimal performance due to the low arithmetic intensity of each gate. Another extreme is to fuse all gates into a single kernel, which would exponentially increase the amount of computation.

To improve simulation performance on GPUs, \Sys uses a dynamic programming algorithm to partition the gates of a stage into kernels.
%
We formulate circuit kernelization as an optimization problem as follows.
%

%% \subsection{Dynamic Programming for Gate Fusion}
%% \label{subsec:dp}

\begin{problem}[Optimal circuit sequence kernelization]

Given a cost function $\Call{Cost}{\cdot}$ that maps one or multiple kernels (a sequence of gates) to their cost (i.e., a real number),
%
the optimal circuit sequence kernelization problem takes as input
%
a quantum circuit $\m{C}$ represented as a sequence of gates,
%
and
%
returns a kernel sequence $\m{K}_0,...,\m{K}_{b-1}$ that minimizes
the total execution cost:
\begin{equation}
\sum_{i=0}^{b-1} \Call{Cost}{\m{K}_i}
\label{eqn:dp_objective}
\end{equation}
such that each kernel consists of a contiguous segment of the gate sequence $\m{C}$.
\label{problem:kernelization}
\end{problem}


% \begin{figure}
%     \centering
%     \subfloat[Sequence\\representation]{
%     \includegraphics[scale=0.5]{figures/sequence.pdf}
%     \label{fig:sequence}
%     }
%     \subfloat[An example state of \Syss dynamic programming.]{
%     \includegraphics[scale=0.5]{figures/dp_state.pdf}
%     \label{fig:dp_state}
%     }
%     \vspace{-1em}
%     \caption{\Cref{fig:sequence} shows a sequence representation for the quantum circuit in \Cref{fig:dp_state}.}
%     \label{fig:my_label}
% \end{figure}


%\UA{The description of the DP algorithm is informal.  We need to do
% more work to get this right, but we do not have time before the
% deadline.  So we are avoiding definitions, etc.}

%% \paragraph{DP state.}
%% \Sys uses a dynamic programming (DP) algorithm to decide how to fuse gates into kernels and how to execute each kernel (e.g., linear or shared-memory kernels).

We note that summing up the cost of individual kernels
(\Cref{eqn:dp_objective}) is a faithful representation of the total
cost, because on a GPU, each kernel may execute in parallel, but
multiple kernels are executed sequentially.
%
%% This is because each kernel updates the entire state vector and
%% therefore cannot be executed in parallel with others.

\subsection{Ordered Kernelizer}
\begin{figure}
%\begin{algorithm}
{
% MX: comment out \small if we have space
\small
\begin{algorithmic}[1]
\Function{$\Call{OrderedKernelizer}{}$}{$\m{C}$}

\State {\bf Input:} A quantum circuit $\m{C}$ represented as a sequence of gates.
\State {\bf Output:} A sequence of kernels.
\State //  $DP[i]$ stores the minimum cost to kernelize the first $i$ gates and the corresponding kernel sequence.

\State $DP[0] = (0, [])$
% \State $Q = \bigcup_{gate \in \m{C}} {qubits(gate)}$
\For {$i = 0$ \textbf{to} $|\m{C}|-1$} 
\State $DP[i+1] = \min_{0 \le j \le i}\{DP[j] + \Call{Cost}{\m{C}[j, \ldots,i]}\}$\label{line:dp-simple-add}
\EndFor
\State \Return $DP[|\m{C}|].kernels$
\EndFunction
\end{algorithmic}
}
%\end{algorithm}
\vspace{-1em}
\caption{The \tcd{OrderedKernelizer} Algorithm.
%The ``+'' operator between $(cost, kernels)$ (the value of $DP[i]$) means adding the cost and concatenating the $kernels$ sequence.
The ``+'' operator in line~\ref{line:dp-simple-add} means adding the cost and appending the kernel to the sequence.
}
\label{alg:dp-simple}
\end{figure}

We first present a dynamic programming (DP) algorithm that solves the
optimal circuit kernelization problem in \Cref{alg:dp-simple}.
The algorithm, called \tcd{OrderedKernelizer}, takes the circuit
representation as a sequence of gates and outputs a sequence of kernels.
%
The \tcd{DP} variable maps a gate (position) in the circuit to a pair
of total cost for the prefix of the circuit up to that gate (excluding
the gate) and sequence of kernels for that prefix.
%
The algorithm starts with a total cost of zero and an empty kernel
sequence.
%
It then considers each possible gate $\m{C}[i]$ in increasing order of $i$ and
computes for that gate the optimal cost.
%
To compute the optimal cost at a position, \tcd{OrderedKernelizer} examines the cost of all possible kernels ending at that position and takes the minimum.
%
Because for each gate, the algorithm considers all possible kernels
ending at that gate, its run-time is asymptotically bounded by the
square of the length of the circuit, i.e., $O(|\m{C}|^2)$.

Although \tcd{OrderedKernelizer} runs in polynomial time, it has a significant limitation: it only considers a specific sequential ordering of the circuit.
%
It is a priori difficult to determine an ordering that yields
the lowest cost. In \Cref{fig:dp_with_optimization}, for example, the optimal kernel sequence might be $\{g_0, g_8, g_9\}, \{g_1, g_2, g_4\}, \{g_3\}, \{g_5, g_6, g_7\}$ if the cost for 4-qubit kernels is much higher than that for smaller kernels. \tcd{OrderedKernelizer} cannot find this kernel sequence if it is not provided with the corresponding ordering of the circuit. On the other hand, it is intractable to consider the exponentially many possible sequences. We present an algorithm to resolve this dilemma, in the next section.


%, but, intuitively, we would like the gates that
%operate on the same qubits close in the sequential order.
%
% In the rest of this section, we present two algorithms to accomplish
% this goal, and evaluate them in \Cref{subsec:eval-dp}.
% %
% The first algorithm applies a heuristic to determine the order and
% operates within the same time complexity as the
% \tcd{OrderedKernelizer} algorithm.\ZJ{Add a sentence to describe the second algorithm}.

% \subsection{Weight-Ordered Kernelizer}
% We present the \tcd{WeightOrderedKernelizer} algorithm, which takes a quantum circuit as an input and generates an ordered sequence representation of the circuit by topologically
% sorting the circuit, while assigning weights (priorities) to gates.
% %
% The algorithm assigns weights to gates such that gates that are close
% in the circuit and operate on ``nearby'' qubits are ordered close
% in the ordered sequence.
% %
% To determine the ordering, the algorithm starts by assigning a weight
% of $0$ to each qubit and orders the gates incrementally as follows.
% \begin{itemize}
% \item Of the gates that come next in the topological sort, select the
%   gate $g$ with the highest average incoming qubit weight;
% \item Multiply the weight of each and every qubit by $0.9$.
% \item Increase the weight of each and every qubit $j$ by $0.5^{|i-j|}$ for each qubit $i$ incident to the gate $g$.
% \end{itemize}
% %

% % \ZJ{It's hard to understand the weight-ordered kernelizer based on the above rules. A concrete example may help. We may also need to add a sentence or two to explain why this strategy can help improve locality.} \MX{Maybe just remove this algorithm. It does not add much to the story.}

% Because each gate is selected once, and the algorithm performs linear
% work in the number of qubits for each selected gate, the total time of
% the algorithm is $O(n|\m{C}|)$ where $n$ is the number of qubits, which is bounded by $O(|\m{C}|^2)$,
% in all but unrealistic circuits.
% %
% Having selected the topological sort of the circuit, the algorithm
% runs the \tcd{OrderedKernelizer} on the topological sort.

\subsection{\Syss Kernelization Algorithm}

To systematically consider multiple sequence permutations at the same time while not expanding the search space exponentially,
we present a key constraint on kernels to \Syss kernelization algorithm in \Cref{alg:dp}.

\begin{constraint}[Constraint on \Syss kernels]
For a kernel $\m{K}$, if there are two gates $\m{C}[j_1], \m{C}[j_2]$ sharing a qubit $q$ such that $j_1 < j_2, \m{C}[j_1] \in \m{K}, \m{C}[j_2] \notin \m{K}$, then $\forall\, k > j_2$, if
\begin{enumerate}
    \item either $q \in \Call{Qubits}{\m{C}[k]}$
    \item or $\exists\, q' \in \Call{Qubits}{\m{C}[k]}$ such that $\not\exists\, j_0 < j_2,\, (\m{C}[j_0] \in \m{K}) \land (q' \in \Call{Qubits}{\m{C}[j_0]})$,
\end{enumerate}
then we constrain that $\m{C}[k] \notin \m{K}$.
\label{dp-constraint}
\end{constraint}

This constraint ensures correctness in \Cref{thm:dp-correct}
while maintaining the result to be at least as good as \tcd{OrderedKernelizer} in \Cref{thm:dp-optimal}. The time complexity will be studied in \Cref{subsec:dp-simplify}.


\begin{figure}
%\begin{minipage}{\textwidth}
%\begin{algorithm}
{
% MX: comment out \small if we have space
\small
\begin{algorithmic}[1]
\Function{$\Call{Kernelize}{}$}{$\m{C}$}

\State {\bf Input:} A quantum circuit $\m{C}$ represented as a sequence of gates.
\State {\bf Output:} A sequence of kernels.
\State // Suppose that we have an ordered kernel set $\KS{}$ in the first $i$ gates, $DP[i,\KS{}]$ stores the minimum cost to kernelize the first $i$ gates \emph{except for the gates in $\KS{}$} and the corresponding kernel sequence.
\State $DP[i,\KS{}] = (\infty, [])$ for all $i, \KS{}$
\State $DP[0,\emptyset] = (0, [])$
% \State $Q = \bigcup_{gate \in \m{C}} {qubits(gate)}$
\For {$i = 0$ \textbf{to} $|\m{C}|-1$} \label{dp:loop_i}
\For {\textbf{each} $\KS{}$ \textbf{such that} $\exists\, \m{K},\,\m{C}[i] \in \m{K}\in \KS{}$ \textbf{and} $\m{K}$ satisfies \Cref{dp-constraint}} \label{dp:loop_ks}
\State {$\tilde{\KS{}} = \KS{} \setminus \{\m{K}\}$}
\If {$|\m{K}|>1$}
\State {$DP[i+1,\KS{}] = DP[i,\tilde{\KS{}} \cup \{\m{K} \setminus \{\m{C}[i]\}\}]$} \label{dp:add-directly}
\Else \ // $\m{K} = \{\m{C}[i]\}$
\State {$DP[i+1,\KS{}] = \displaystyle\min_{\KS{}' \supseteq \tilde{\KS{}}}\left\{DP[i,\KS{}'] + \Call{Cost}{\KS{}'\setminus\tilde{\KS{}}}\right\}$} \label{dp:singleton-kernel}
\EndIf
\EndFor
\EndFor
\State $ DP_{best} = \min_{\KS{}}\left\{DP[|\m{C}|,\KS{}]+\Call{Cost}{\KS{}}\right\}$ \label{dp:compute_f_best}
\State \Return $DP_{best}.kernels$
\EndFunction
\end{algorithmic}
}
%\end{algorithm}
%\end{minipage}
\vspace{-1em}
\caption{\Syss kernelization algorithm.
The ``+'' operators in lines~\ref{dp:singleton-kernel} and~\ref{dp:compute_f_best} mean adding the cost and appending the kernel set to the sequence. %The order of the kernels in the kernel set is maintained in place (replacing $\m{K} \setminus \{\m{C}[i]\}$ with $\m{K}$ in line~\ref{dp:add-directly}).
We move $\m{K}$ to the end in the kernel set whenever the gate pair $\m{C}[j_1], \m{C}[j_2]$ in \Cref{dp-constraint} does not exist for $\m{K}$ in~\ref{dp:add-directly}, or maintain the order in place (replacing $\m{K} \setminus \{\m{C}[i]\}$ with $\m{K}$) otherwise. %\MX{I don't want to introduce "open kernels" and "absorbing kernels" here. In fact, open kernels must come after absorbing kernels. If the gate pair $\m{C}[j_1], \m{C}[j_2]$ in \Cref{dp-constraint} does not exist, we know the kernel is an open kernel, and it may make some of the other kernels absorbing kernels, so it's always safe to move it to the end. If it exists, we know it's an absorbing kernel, so it's always safe to maintain the order in place. However, we do not have a way to combine these two cases.}
We require $\tilde{\KS{}}$ to be a suffix of $\KS{}'$ in line~\ref{dp:singleton-kernel}.}
\label{alg:dp}
\end{figure}


%\begin{lemma}
%If a kernel $\m{K}$ satisfies \Cref{dp-constraint} with respect to $\m{C}$, it also satisfies \Cref{dp-constraint} with respect to any subsequence $\m{C}'$ of $\m{C}$ as long as $\m{C}'$ still contains all gates in $\m{K}$.
%\label{lemma:constraint-subseq}
%\end{lemma}
\begin{theorem}[Correctness of \Syss kernelization algorithm]
%If all kernels satisfy \Cref{dp-constraint}, are subsequences of $\m{C}$, and are sorted by the largest gate index in $\m{C}$, concatenating the kernels forms a sequence $\m{C}'$ which is topologically equivalent to $\m{C}$. 
\Syss kernelization algorithm in \Cref{alg:dp} returns a kernel sequence such that concatenating the kernels forms a sequence topologically equivalent to $\m{C}$. 
\label{thm:dp-correct}
\end{theorem}

\begin{proof}
%C'[j'1] C'[j'2] C'[j'3] C'[i']
%C[i]         C[j]
%Let us keep adjusting $\m{C}'$ to make the common prefix with $\m{C}$ longer.
%Suppose the first gate index where $\m{C}'$ and $\m{C}$ differ is $i$, and $\m{C}[i] = \m{C}'[i'] \in \m{K}_t$. 
%Because this is the first difference, we have $i' > i$. Consider each gate $\m{C}'[j']$ such that $i \le j' < i'$ and the corresponding gate $\m{C}[j]$, we have $j > i$. Because $\m{K}_t$ is a subsequence of $\m{C}$, $\m{C}'[j']$ appears before $\m{C}'[i']$ in $\m{C}'$ but $\m{C}[j]$ appears after $\m{C}[i]$ in $\m{C}$, $\m{C}[j] \notin \m{K}_t$.
%Now apply \Cref{dp-constraint} on $i, j$ and $\m{K}_t$, 
%Proof by induction on the number of kernels. If there is only one kernel, the statement is trivial. Otherwise, consider the kernel $\m{K}$ containing $\m{C}[|\m{C}|-1]$ and the largest index $j_0$ such that $\m{C}[j_0] \neq \m{C}'[j_0]$, then $j_0 < \m{C}-1$ because the kernel containing $\m{C}[|\m{C}|-1]$ is ordered the last in $\m{C}'$. If $\m{C}[j_0]\notin \m{K}$, we can remove this kernel from both $\m{C}$ and $\m{C}'$, and apply the induction hypothesis. Otherwise, suppose $\m{C}'[j_0] = \m{C}[i]$, then $i < j_0$.
%We can then apply \Cref{dp-constraint} on $\m{K}$ for each $j = i + 1, \dots, j_0$ by \Cref{lemma:constraint-subseq}. Because $\m{K}$ is a subsequence of $\m{C}$, $\m{C}[j] \notin \m{K}$. 
%$\m{C}[k] \in \m{K}$, either $\Call{Qubits}{\m{C}[i]} \cap \Call{Qubits}{\m{C}[j]} = \emptyset$, or 
%
%
Proof by induction on $i$ that for each $DP[i,\KS{}].cost < \infty$, appending $\KS{}$ to $DP[i,\KS{}].kernels$ results in sequence $\m{C}_{\KS{}}^i$ which is topologically equivalent to a the sequence $\m{C}[0], \m{C}[1]$, $\dots, \m{C}[i-1]$ (denote this sequence $\m{C}^i$). This holds for $i = 0$ where $DP[i,\emptyset].kernels$ and $\m{C}^0$ are both empty.

Suppose the induction hypothesis holds for $i$. For $i+1$, for any $\m{K}$ satisfying \Cref{dp-constraint}, if $|\m{K}| = 1$, line~\ref{dp:singleton-kernel} in the algorithm makes the order of appending $\KS{}$ to $DP[i+1,\KS{}].kernels$ the same as the order of appending $\KS{}'$ to $DP[i,\KS{}'].kernels$ for some $\KS{}'$ when $\tilde{\KS{}}$ is a suffix of $\KS{}'$, so we can directly apply the induction hypothesis to prove it for $i+1$.

If $|\m{K}| > 1$, line~\ref{dp:add-directly} inserts $\m{C}[i]$ to the end of $\m{K}$ in $\m{C}_{\KS{}}^i$ when the gate pair $\m{C}[j_1], \m{C}[j_2]$ exists in \Cref{dp-constraint}. If there is a gate $\m{C}[j_2']$ after the last gate of $\m{K}$ in the original sequence $\m{C}_{\KS{}}^i$ which shares a qubit $q$ with $\m{C}[i]$, from the constraint for each $j_1'$,
\begin{enumerate}
    \item $q \notin \Call{Qubits}{\m{C}[j_1']}$ for any $\m{C}[j_1'] \in \m{K}$;
\end{enumerate}
from the fact that the gate pair $\m{C}[j_1], \m{C}[j_2]$ exists,
\begin{enumerate}
\item[2.] $\exists\, j_0 < j_2 < j_2', (\m{C}[j_0] \in \m{K}) \land (q \in \Call{Qubits}{\m{C}[j_0]}$.
\end{enumerate}
These two conditions conclude that such a gate does not exist, and we can safely insert $\m{C}[i]$ to the end of $\m{K}$ in $\m{C}_{\KS{}}^i$ without breaking the topological equivalence.

%moves $\m{K} \setminus \{\m{C}[i]\}$ to the end (and then replace it with $\m{K}$), and we need to prove this move maintains topological equivalence. Let $j_1$ be the first gate in $\m{K}$. % If $\m{K} \setminus \{\m{C}[i]\}$ is not already at the end of $\tilde{\KS{}} \cup \{\m{K} \setminus \{\m{C}[i]\}\}$ in $DP[i, \cdot]$
%For each kernel $\m{K}'$ after $\m{K} \setminus \{\m{C}[i]\}$ in $\tilde{\KS{}} \cup \{\m{K} \setminus \{\m{C}[i]\}\}$, there exists $j_1 < j_2 < i$ such $\m{C}[j_1] \in \m{K}$, $\m{C}[j_2] \in \m{K}'$. These $\m{C}[j_2]$ gates are the only gates that could break the topological equivalence (in $\m{C}^i$, $\m{C}[j_1]$ is before $\m{C}[j_2]$, but we are going to reverse this order in $\m{C}_{\KS{}}^{i+1}$. 
%
%Let $\m{C}[j_1]$ be the last gate in $\m{K}$ before $\m{C}[i]$. If $j_1 = i - 1$, the induction hypothesis holds for $i+1$. Otherwise, for each $j_2 > j_1$, we apply \Cref{dp-constraint} to $\m{K}$. If $\m{C}[j_2]$

When the gate pair $\m{C}[j_1], \m{C}[j_2]$ does not exist in \Cref{dp-constraint}, line~\ref{dp:add-directly} moves $\m{K}$ to the end of $\m{C}_{\KS{}}^i$. For each gate $\m{C}[j_1']$ in $\m{K}$, for each gate $\m{C}[j_2']$ not in $\m{K}$ after $\m{C}[j_1']$ in the original sequence $\m{C}_{\KS{}}^i$, $\m{C}[j_1']$ and $\m{C}[j_2']$ do not share any qubits. So we can safely move the entire kernel $\m{K}$ to the end without breaking the topological equivalence.

In all cases, we have proved that $\m{C}_{\KS{}}^{i+1}$ is topologically equivalent to $\m{C}^{i+1}$. So $\m{C}_{\KS{}}^{|\m{C}|}$ is topologically equivalent to $\m{C}^{|\m{C}|}$, which proves that any state in line~\ref{dp:compute_f_best} in the algorithm returns a kernel sequence such that concatenating the kernels forms a sequence topologically equivalent to $\m{C}$.
\end{proof}

\begin{theorem}[\Cref{dp-constraint} allows all contiguous kernels]
Any kernel of a contiguous segment of the gate sequence $\m{C}$ satisfies \Cref{dp-constraint}. \label{thm:contiguous}
\end{theorem}
\begin{proof}
For any kernel $\m{K}$ of a contiguous segment of gates, for any $j_1 < j_2 < k$ such that $\m{C}[j_1] \in \m{K}, \m{C}[j_2] \notin \m{K}$, we know that $\m{C}[k] \notin \m{K}$ by contiguity.
\end{proof}

%\ZJ{The statement in \ref{thm:dp-optimal} does sound that it discovers a global optimal solution. How about: \Syss kernelization algorithm in \Cref{alg:dp} returns an {\em optimal} kernel sequence that minimizes its total execution cost defined by \Cref{eqn:dp_objective}.}
%\MX{It does not discover a global optimal, nor does it return an optimal kernel sequence. It is just at least as good as the \tcd{OrderedKernelizer} algorithm.}

\begin{theorem}[\Syss kernelizer is at least as good as \tcd{OrderedKernelizer}]
\Syss kernelizer in \Cref{alg:dp} always returns a kernel sequence with a total execution cost no more than \tcd{OrderedKernelizer}, which is optimal for \Cref{problem:kernelization}. \label{thm:dp-optimal}
\end{theorem}

%\begin{wrapfigure}{r}{0.45\textwidth}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/kernelizer_state.png}
    \caption{An example DP state in \Syss implementation. In this figure, $\m{C}[i]$ is denoted by $g_i$.}
    \vspace{-1em}
    \label{fig:dp_with_optimization}
\end{figure}

\ifarxiv
The proof is provided in the appendix for brevity.
\else
The proof is provided in the supplemental text for brevity.
\fi

% %
% The algorithm maintains a set of kernels along with a set of
% \defn{extensible qubits} for each kernel. 
% Extensible qubits are qubits that can be connected to another
% gate without breaking the convexity of the kernel and without creating cyclic dependencies between kernels. 
% %
% The DP algorithm represents a circuit as a sequence of gates that
% matches a topological sort of gates in the circuit.
% %
% For example, \Cref{fig:sequence} shows a valid sequence representation for the quantum circuit in \Cref{fig:dp_state}.
% %

% Given a circuit represented as a sequence of gates, the DP algorithm,
% shown in \Cref{alg:dp}, starts by initializing the DP state, and adding the gates of the circuit one by one in
% the increasing order.
% % 
% The DP state is indexed by a position $i$ (starting from zero) and a
% kernel set $\KS{}$ at that position; it maps the position and the kernel
% set to a cost (a real number) and a set of \defn{closed kernels} up to that position. Closed kernels are kernels with no extensible qubits, so we cannot add any gates to them.
% The DP state represents the best kernelization solution containing the kernel set $\KS{}$ up to position $i$: the closed kernels represent the best kernelization of the first $i$ gates excluding $\KS{}$, and the cost of the DP state is the total cost of closed kernels.
% %


% \Cref{fig:dp_state} shows an example DP state $(i, \KS{})$ with $i = 7$ and $\KS{} = \{\m{K}_1, \m{K}_2\}$. 
% Note that the extensible qubit set for $\m{K}_1$ only includes $q_3$, since we can only add future gates operating on $q_3$ (e.g., $g_8$) into $\m{K}_1$. Adding a gate operating on other qubits (e.g., $g_7$ on $q_1$ and $q_2$) into $\m{K}_1$ violates the convexity of the kernel $\m{K}_1$. 
% Note that $\KS{}$ does not include kernels with no extensible qubits (e.g., the kernel for $g_0$ and $g_1$ is not in $\KS{}$), this is because we cannot add any future gates into a kernel with no extensible qubits. This simplification helps us reduce the complexity of the DP algorithm.


% % To add a gate to the DP state, the algorithm considers each kernel
% % state set $\KS{}$ and updates the kernels and their state by
% % considering the impact of the gate to each kernel.
% % %
% % Specifically, there are three cases.  
% % %
% % In the first case, the gate lies an non-extensible qubit and therefore
% % the kernel remains unaffected by this gate.
% % %
% % In the second case, ...
% % %
% % In the third case, ..

% To add the $i$-th gate $\m{C}[i]$, the algorithm considers each DP state $(i,\KS{})$ and updates the DP state by considering the
% impact of the gate on each kernel.
% %
% When adding a gate, there are two possibilities:
% %
% The first is to create a singleton kernel consisting of the gate
% (Lines~\ref{dp:new_kernel_begin}--\ref{dp:new_kernel_end} in
% \Cref{alg:dp}).
% %
% The second is to add the gate to an existing kernel, if all input
% qubits of the gate are extensible
% (Lines~\ref{dp:existing_kernel_begin}--\ref{dp:existing_kernel_end} in
% \Cref{alg:dp}).
% %
% In either case, we check if any kernel's extensible qubit set becomes empty after adding the gate, \emph{close} such kernels, and record their costs.
% In each case, we update the extensible qubit set for each kernel state
% after adding the gate by checking if there will be no feasible
% schedules for all kernels in $\KS{}$ if we append a single-qubit gate
% for each qubit (line~\ref{dp:feasible_schedule}); more details on this
% will be described in \Cref{subsec:dp_optimizations}.  We then
% \emph{close} the kernels with empty extensible qubit sets
% (line~\ref{dp:close_begin} to line~\ref{dp:close_end}) and record
% their cost (line~\ref{dp:record_cost}).


% \MX{This is the definition, not property}
% \begin{theorem}
% For a circuit with sequence representation $L=(g_0,g_1,...,g_{m-1})$ and a kernel state \KS{} with fused gates $\m{G}'$ and extensible qubits $\m{X}'$ at the $(i-1)$-th iteration, we can fuse $g_i$ into the kernel if and only if $g_i$'s qubits are a subset of $\m{X}'$.
% \end{theorem}

\subsection{Reducing Number of DP States}
\label{subsec:dp-simplify}
In a quantum circuit, the number of gates is typically orders of magnitude more than the number of qubits.
Therefore, instead of tracking the gates for each kernel in \Cref{alg:dp}, \Sys maintains the qubit set as well as an \defn{extensible qubit set} for each kernel. %The extensible qubit set is a characterization of \Cref{dp-constraint}.

%As described in \Cref{subsec:dp-cost}, maintaining the qubit set is sufficient to maintain the cost for each kernel. We now show that maintaining these two sets is sufficient to implement \Cref{dp-constraint}.
\begin{definition}[Extensible Qubit for a kernel]
For a kernel $\m{K}$, a qubit $q'$ is extensible at position $i$ if and only if there do not exist two gates $\m{C}[j_1], \m{C}[j_2]$ sharing a qubit $q$ such that $j_1 < j_2 < i, \m{C}[j_1] \in \m{K}, \m{C}[j_2] \notin \m{K}$, and
\begin{enumerate}
\item either $q = q'$
\item or $\not\exists\, j_0 < j_2,\, (\m{C}[j_0] \in \m{K}) \land (q' \in \Call{Qubits}{\m{C}[j_0]})$,
\end{enumerate}
\label{def:extensible-qubit}
\end{definition}
This definition is a direct characterization of \Cref{dp-constraint}: adding the gate $\m{C}[i]$ to a kernel $\m{K}$ satisfies \Cref{dp-constraint} if and only if all qubits of $\m{C}[i]$ are extensible for $\m{K}$ at position $i$. For example, the extensible qubit set is $\{q_5\}$ for the kernel $\m{K}_3$ in \Cref{fig:dp_with_optimization} at the current position -- we can only add gates operating only on this qubit to $\m{K}_3$ to satisfy \Cref{dp-constraint}. 

\ZJ{I find it's hard to understand the definition of extensible qubits based on the above definition. Consider include an example or add a few sentences to explain the intuition behind the definition.}
\MX{It's just constraint 1.}

\MX{Definition and Constraint seem to be in two different systems -- the fonts are different and the numbers are different. Do we want to make them the same?}
\ZJ{That's probably fine if we only have a single constraint in the paper (I didn't find constraint 2).}

\begin{figure}
%\begin{minipage}{\textwidth}
%\begin{algorithm}
{
% MX: comment out \small if we have space
\small
\begin{algorithmic}[1]
\State // $\m{C}[i] \in \m{K}\in \KS{}$
\If{$\m{K} = \{\m{C}[i]\}$} // a new kernel
\State $\Call{ExtensibleQubits}{\m{K},i+1} = \Call{AllQubits}{}$
\Else
\State $\Call{ExtensibleQubits}{\m{K},i+1} = \Call{ExtensibleQubits}{\m{K},i}$
\EndIf
\For{$\m{K}' \in (\KS{} \setminus \m{K})$}
\If {$\Call{ExtensibleQubits}{\m{K}',i} = \Call{AllQubits}{}$} \label{extensible:if-all}
\If{$\m{C}[i] \cap \Call{Qubits}{\m{K}'} \neq \emptyset$} \label{extensible:intersect}
\State $\Call{ExtensibleQubits}{\m{K}',i+1} = 
\Call{Qubits}{\m{K}'} \setminus \Call{Qubits}{\m{C}[i]}$ \label{extensible:qubits-k}
\Else
\State $\Call{ExtensibleQubits}{\m{K}',i+1} = \Call{AllQubits}{}$
\EndIf
\Else
\State $\Call{ExtensibleQubits}{\m{K}',i+1} = \Call{ExtensibleQubits}{\m{K}',i} \setminus \Call{Qubits}{\m{C}[i]}$ \label{extensible:remove-qubits}
\EndIf
\EndFor
\end{algorithmic}
}
%\end{algorithm}
%\end{minipage}
\vspace{-1em}
\caption{Maintaining the extensible qubit set for each kernel after each iteration of the for loop in line~\ref{dp:loop_ks} of \Cref{alg:dp}.}
\label{alg:extensible}
\end{figure}



We append the code fragment in \Cref{alg:extensible} to the end of each iteration of the for loop in line~\ref{dp:loop_ks} of \Cref{alg:dp} to maintain the extensible qubit set for each kernel. \Cref{thm:extensible-correct} ensures the correctness of this approach, and the proof is provided in the %
\ifarxiv
appendix.
\else
supplemental document.
\fi

\begin{theorem}
\Cref{alg:extensible} correctly computes the extensible qubit set for each kernel.
\label{thm:extensible-correct}
\end{theorem}

Because we cannot add any gates to kernels with an empty extensible qubit set like $\m{K}_2$, we compute their cost and remove them from $\KS{}$ in line~\ref{dp:singleton-kernel} of \Cref{alg:dp}.
Because line~\ref{extensible:qubits-k} of \Cref{alg:extensible} restricts the extensible qubit set to be a subset of the qubit set of $\m{K}'$, we do not need to keep track of the qubit set anymore because it is no longer going to be changed. With these optimizations, we present the time complexity for the algorithm.
%
Note that in addition to the two qubit sets, we need an extra boolean variable for the type of each kernel (fusion or shared-memory) to maintain the cost in \Cref{subsec:dp-cost}.

\begin{theorem}
% a(n+1)=a(n)+sum_{i=0}^{k-1} a(n-i) * 2 * \binom{n}{i}
With the extensible qubit sets maintained in \Cref{alg:extensible}, \Syss kernelization algorithm runs in $O\left(\left(\frac{3.2 n}{\ln{n}}\right)^n \cdot |\m{C}|\right)$ where $n$ is the number of qubits.
\label{thm:dp-complexity}
\end{theorem}
\begin{proof}
For each iteration $i$ in \Cref{alg:dp}, let us compute the maximum number of kernel sets $\KS{}$ that \Sys must consider.

We observe that if we consider the qubit set for each kernel with the extensible qubit set being all qubits, and the extensible qubit set for other kernels, any two of these sets do not intersect. This can be proven by induction on $i$ and the fact that whenever we add $\Call{Qubits}{\m{C}[i]}$ to $\m{K}$, we effectively remove these qubits from all other sets.

% For any two kernels $\m{K}_1, \m{K}_2 \in \KS{}$, if both extensible qubit sets are all qubits, we have $\Call{Qubits}{\m{K}_1} \cap \Call{Qubits}{\m{K}_2} = \emptyset$ by \Cref{dp-constraint}. If one of the extensible qubit sets is all qubits (say $\m{K}_1$), we have $\Call{Qubits}{\m{K}_1} \cap \Call{ExtensibleQubits}{\m{K}_2} = \emptyset$
Because kernels with empty extensible qubit sets are removed from $\KS{}$, there are at most $n$ kernels in $\KS{}$ and the number of ways to partition all qubits into disjoint qubit sets is at most the Bell number $B_{n+1}$, which is less than $\left(\frac{0.792(n+1)}{\ln(n+2)}\right)^{n+1}$~\cite{berend_improved_2010}. Each qubit set can be either the qubit set or the extensible qubit set of a kernel, so we need to multiply this number by at most $2^n$; each kernel can be either fusion or shared-memory, so we need to multiply this number by another $2^n$.
With the extensible qubit sets maintained, the order of kernels does not affect the DP transitions, so the number of different kernel sets is at most $4^n B_{n+1}$.
Each iteration of the for loop in line~\ref{dp:loop_ks} of \Cref{alg:dp} takes polynomial time, so the time per iteration $i$ is at most $O\left(\left(\frac{3.2 n}{\ln{n}}\right)^n\right)$. There are $|\m{C}|$ iterations, so the total time complexity is $O\left(\left(\frac{3.2 n}{\ln{n}}\right)^n \cdot |\m{C}|\right)$.
\end{proof}

Although the time complexity is superpolynomial, $|\m{C}|$ can also be superpolynomial to $n$. The algorithm may even run faster than \tcd{OrderedKernelizer} if $|\m{C}| = \Omega\left(\left(\frac{3.2 n}{\ln{n}}\right)^n\right)$.

%By only keeping track of two qubit sets instead of the gates in each kernel, this approach significantly simplifies the representation of a DP state and reduces the number of DP states \Sys considers.


% All qubits are extensible for $\m{K}$ at the position of the first gate of $\m{K}$. To maintain the extensible qubit set, we note that if $\m{C}[i] \in \m{K}$, the extensible qubit set at position $i + 1$ is the same as position $i$; if $\m{C}[i] \notin \m{K}$, for each qubit $q'$, $q'$ is extensible at position $i + 1$ if and only if $q'$ is extensible at position $i$ and there does not exist a gate $\m{C}[j_1]$ sharing a qubit $q$ with $\m{C}[i]$ such that $j_1 < i, \m{C}[j_1] \in \m{K}$, and
% \begin{enumerate}
% \item $q = q'$
% \item or $\not\exists\, j_0 < i,\, (\m{C}[j_0] \in \m{K}) \land (q' \in \Call{Qubits}{\m{C}[j_0]})$,
% \end{enumerate}
% by \Cref{def:extensible-qubit}. So an extensible qubit $q'$ for $\m{K}$ at position $i$ becomes not extensible at position $i+1$ if and only if $\m{C}[i] \notin \m{K}$, and either
% \begin{enumerate}
% \item $(\Call{Qubits}{\m{K}} \cap \Call{Qubits}{\m{C}[j_i]} \neq \emptyset) \land (q' \notin \Call{Qubits}{\m{K}})$
% \item or $(\Call{ExtensibleQubits}{\m{K}} \cap \Call{Qubits}{\m{C}[j_i]} \neq \Call{Qubits}{\m{C}[j_i]}) \land (q' \in \Call{Qubits}{\m{C}[j_i]})$.
% \end{enumerate}
% In this way, we do not need to keep track of the gates in each kernel.


\subsection{Cost Function}
\label{subsec:dp-cost}
The cost function used in \Cref{eqn:dp_objective} should faithfully represent the running time for each kernel. Inspired by HyQuas~\cite{chen2021hyquas}, \Sys considers two approaches to executing each kernel:
\begin{enumerate}
\item \defn{Fusion}: Fuse all gates in a kernel into a single gate by pre-computing the product of the gate matrices and executing that single gate using cuQuantum~\cite{bayraktar_cuquantum_2023}. The cost depends solely on the number of qubits in the kernel. %\MX{Not sure if here is the correct place to say we use cuQuantum} \SC{I feel we can say it here}
\item \defn{Shared-memory}: Load the state vector into GPU shared memory in batches and execute the gates one by one instead of fusing them to a single matrix. The cost can be approximated as $\alpha + \sum_{g\in \m{K}} \Call{Cost}{g}$, where $\alpha$ is a constant that corresponds to the time to load a micro-batch of state coefficients into GPU shared memory, and $\Call{Cost}{g}$ is the cost to simulate the application of the gate $g$ in the GPU shared memory.
This corresponds to \tcd{SHM-GROUPING} in HyQuas.
\end{enumerate}
%Either way, we do not need to keep track of all previous gates when we add a gate into a kernel and update the cost if we maintain the qubit set of a kernel. This opens up optimization opportunities for the implementation of the kernelization algorithm.

\subsection{Other Optimizations to the DP Algorithm}
\label{subsec:dp_optimizations}

%\ZJ{I like the new outline for presenting the DP algorithm (i.e., first claiming its optimality and then introducing a set of optimizations to reduce its run time). At the end of this subsection, it would be helpful to add a discussion on what optimizations preserve optimality and what does not. I would assume only a few optimizations do not, right?}

\if 0
The DP algorithm presented in \Cref{alg:dp} can discover an optimal strategy to kernelize a circuit but is prohibitively expensive to run in practice. This section describes a list of optimizations in \Sys to accelerate the DP algorithm.

\paragraph{Extensible and fixed kernels.}
Tracking the set of extensible qubits for each kernel is expensive. 
One way to simplify the computation of extensible qubits is to maintain a total order for all kernels in $\KS{}$; however, doing so will result in significantly more DP states since different orders of the same set of kernels will be in different DP states. 
Thus, \Sys categorizes kernels into \defn{extensible} and \defn{fixed} kernels, and maintains an order for {\em fixed} kernels in the DP state. 

\begin{definition}[Extensible and fixed kernels]
A kernel $\m{K}$ is extensible if its extensible qubit set is all qubits; otherwise, it is fixed.
\end{definition}

\Cref{fig:dp_with_optimization} shows an example DP state with extensible and fixed kernels. \Sys requires that all extensible kernels are scheduled after fixed kernels (explained later), therefore $\KS{}$ must begin with $\m{K}_2, \m{K}_3$.
By definition, extensible kernels (e.g., $\m{K}_1$ and $\m{K}_4$) do not have any dependencies between each other, which allows them to be scheduled in an arbitrary order after all fixed kernels.

This order for fixed kernels makes it easy to compute the extensible qubit set for each kernel: whenever we add a gate $g$ to a kernel $\m{K}$, we simply remove $g$'s qubits from all extensible qubit sets of kernels before $\m{K}$ in $\KS{}$. 
For the example DP state in \Cref{fig:dp_with_optimization}, (1) adding $g_8$ to an extensible kernel (e.g., $\m{K}_1$ or $\m{K}_4$) will remove $q_2$ and $q_3$ from the extensible qubit sets of all fixed kernels (i.e., $\m{K}_2$ and $\m{K}_3$), (2) adding $g_8$ to $\m{K}_3$ will remove $q_2$ and $q_3$ from the extensible qubit set of $\m{K}_2$, and (3) adding $g_8$ to $\m{K}_2$ does not require updating the extensible qubit set for any kernels since $\m{K}_2$ is the first fixed kernel.
%%%
To avoid introducing cyclic dependencies, we refrain from changing the qubit set of any fixed kernels (another reason why these kernels are fixed).



\ZJ{To be removed <===============}
Checking if we can add a gate to a kernel on the fly (Line~\ref{dp:check_gate} in \Cref{alg:dp}) is expensive, and maintaining the extensible qubit set for each kernel is also expensive. If we maintain an order of the kernels, maintaining the extensible qubit set will only take linear time on the number of qubits for each kernel.
However, maintaining a strict order of kernels in $\KS{}$ would greatly restrain the representability of the DP state; therefore, we compromise by categorizing the kernels into \defn{extensible kernels} and \defn{fixed kernels}.

\begin{definition}[Extensible and fixed kernels]
A kernel $\m{K}$ is extensible if its extensible qubit set is all qubits; otherwise, it is fixed.
\end{definition}

Extensible kernels do not have any dependency on each other. They can be placed arbitrarily in an order of kernels in $\KS{}$ as long as all extensible kernels are placed at the end.

As long as newly added gates do not change any qubit set of kernels of fixed kernels (therefore not creating any new dependencies -- this is why it is called \emph{fixed}), we are able to maintain an order of the kernels in $\KS{}$ where all extensible kernels are placed at the end.

After the order is determined, it will be easy to maintain the extensible qubit set for each kernel: whenever we add a gate to a kernel $\m{K}$, simply remove the gate's qubits from all extensible qubit sets of kernels before $\m{K}$.

\ZJ{=========>}
\fi

\paragraph{\Kwins{} qubits.}
Recall that \Syss circuit partitioner allows mapping the insular qubits of a gate to regional and global qubits. 
Before loading a batch of states to GPU, the values of all global and regional qubits for the batch are known, which are leveraged by \Sys to simplify computation.
Specifically, for gates with \kwins{} non-local qubits, \Sys retrieves the non-local qubits' values and converts these gates into local gates with fewer qubits.

We can do more along this line for shared-memory kernels. A physical qubit is \defn{active} for a shared-memory kernel if its states are loaded into the shared memory in a single micro-batch. 
For \emph{non-active} local qubits, \Sys applies a similar optimization to gates with \kwins{} non-active local qubits that converts these gates into smaller gates with only active qubits.
%%%
Because we can swap two adjacent gates if all qubits they share are \kwins{} to both gates, we can slightly lift the \Cref{dp-constraint} by ignoring any qubit in line~\ref{extensible:intersect} of \Cref{alg:extensible} that is \kwins{} to $\m{C}[i]$ and all gates in $\m{K}'$. In order to know this, we additionally maintain an active qubit set for each shared-memory kernel $\m{K}'$ for the \kwnonins{} qubits of all gates in $\m{K}'$.

Furthermore, we additionally maintain an extensible \kwins{} qubit set that is maintained in the same way as the extensible qubit set in line~\ref{extensible:remove-qubits} of \Cref{alg:extensible} but initialized as 
$\Call{ExtensibleInsularQubits}{\m{K}',i+1} = \Call{AllQubits}{} \setminus \Call{Qubits}{\m{C}[i]}$ in line~\ref{extensible:qubits-k} of \Cref{alg:extensible}. We can then further lift the \Cref{dp-constraint} by allowing to add a gate $\m{C}[i]$ to a shared-memory kernel $\m{K}'$ as long as its \kwins{} qubits are in the extensible \kwins{} qubit set and its \kwnonins{} qubits are in the extensible qubit set.

%\begin{wrapfigure}{r}{0.45\textwidth}
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/swap_cx0.pdf}
    \vspace{-1em}
    \caption{If we swap an $X$ gate with an adjacent $CX$ gate, we need to flip the control state of the new $CX$ gate to $\ket{0}$.}
    \vspace{-1em}
    \label{fig:swap}
\end{figure}
%\end{wrapfigure}

After the DP algorithm, we reconstruct the topological order to see which gates are swapped. If one of the gates being swapped is anti-diagonal (e.g., the $X$ gate) and the other gate is a control gate, \Sys flips the control state of that gate, as shown in \Cref{fig:swap}.

This optimization opens up more ways to reorder the circuit sequence.

% \ZJ{This seems like implementation details. I would suggest we remove this paragraph.} \Sys also attaches a gate if it has exactly one local qubit. 
% If there is no other gate on the local qubit in this stage, we first try to attach the gate to a gate in the next stage if this gate still has exactly one local qubit in the next stage, and simply keep the gate if it cannot find a good place to attach.


%on each qubit is a common pattern at the beginning of some circuits. They cause an exponential blowup in the number of different DP states.
%Note that there should not be any qubit with only single-qubit gates (otherwise the qubit is not entangled in the circuit), we attach each single-qubit gate to an adjacent multi-qubit gate.

%If a single-qubit gate's qubit is non-\kwins{}, we need to mark the corresponding qubit in the multi-qubit gate it attaches to as non-\kwins{}.

%If both the single-qubit gate's qubit and the corresponding qubit in the adjacent multi-qubit gate are \kwins{} (the corresponding qubit in the multi-qubit gate should be a control qubit here), we can swap these two gates instead of attaching without affecting the execution result, making the single-qubit gate possible to be merged with some other single-qubit gates on the same qubit. Note that as shown in \Cref{fig:swap}, if the single-qubit gate's matrix is anti-diagonal (e.g., the $X$ gate), we need to flip the control state of the corresponding control qubit of the multi-qubit gate -- if the control state was $\ket{1}$, we need to flip it to $\ket{0}$ after swapping.


%\ZJ{@mingkuan: I rewrote this paragraph and dropped some details. Take a look and let me know if you think some details are important and must be mentioned here.}

\if 0
\MX{The following is wrong and misses important details. Fixed fusion kernels and fixed shared-memory kernels are very different. We need to keep track of one set which is the intersection of the kernel's qubits and the extensible qubit set for both kernels, but we need to keep track of an additional set which is the extensible qubit set for shared-memory kernels. This is also why I put "Insular qubits and shared-memory kernels" before this paragraph -- that optimization affects this which causes significant changes in the index of DP states. So I don't think we can leave that in the implementation details.}
\ZJ{I see. I moved the insular qubit part back to this section.}
%Therefore, instead of tracking a gate set for each kernel, \Sys maintains the kernel type (i.e., fixed or extensible) and its set of qubits. For each fixed kernel, \Sys also tracks its set of extensible qubits, which is a subset of its qubit set. 
%This approach significantly reduces the number of DP states \Sys considers.

\ZJ{Old version <=========}
\paragraph{Maintaining the minimum necessary for the cost function}
Recall that $\Call{Cost}{\cdot}$ maps a kernel to its cost, which requires keeping all the gates in a kernel. However, the number of gates can be much more than the number of qubits, and keeping them may cause the DP state to be too large.

In our implementation, the cost of a \defn{fusion kernel} (computing the unitary matrix representation of the kernel) is only related to the number of qubits in the kernel, and the cost of a \emph{shared-memory kernel} is a constant number for the initialization cost plus a cost for each gate (which can vary for different types of gates). Therefore, we keep track of the type for each kernel at the beginning, and we only need to keep track of the qubit set (which is also necessary to the DP itself). Whenever we add a gate to a shared-memory kernel, we record the cost of the gate immediately instead of when recording the cost of the kernel.

We do not keep track of extensible qubit sets for extensible kernels because they are defined to be all qubits. When we generate a fixed kernel, we need to keep track of its extensible qubit set; but recalling that newly added gates cannot change any qubit set of kernels of fixed kernels, we only need to keep track of the intersection of the extensible qubit set and the qubit set of the kernel, which is much smaller and is essentially the qubit set excluding the qubits in the gate which caused the generation of the fixed kernel. For a fixed shared-memory kernel, however, we still need to compute its extensible qubit set: we need to keep track of this set in order to place \kwins{} qubits.

We record the cost of a kernel when generating the fixed kernel because its cost will not change anymore for fusion kernels and its initialization cost will not change anymore for shared-memory kernels. We simply remove a fixed kernel when its qubit set becomes empty.
\ZJ{=========>}
\fi 

\paragraph{Optimizing DP transition.}
When a new gate $\m{C}[i]$ can be subsumed by an existing kernel $\m{K}$ or vice versa, i.e., $\Call{Qubits}{\m{C}[i]} \subseteq \Call{Qubits}{\m{K}}$ or $\Call{Qubits}{\m{K}} \subseteq \Call{Qubits}{\m{C}[i]}$ (and $\Call{Qubits}{\m{C}[i]} \subseteq \Call{ExtensibleQubits}{\m{K}}$ by \Cref{dp-constraint}),
\Sys directly adds $\m{C}[i]$ into $\m{K}$. In other words, \Sys will not consider any $\KS{}$ where $\m{C}[i] \in \m{K}' \in \KS{}$ for any $\m{K}' \neq \m{K}$.
For example, in \Cref{fig:dp_with_optimization}, \Sys will directly add $g_7$ into $\m{K}_4$ without considering other options.
This optimization greatly reduces the amount of DP transitions \Sys must explore.

\paragraph{Deferring adding gates to extensible kernels.}
To further reduce the number of DP states, we keep gates as single-gate kernels when their extensible qubit sets are all qubits instead of trying to add them to each of the kernels. Upon running line~\ref{extensible:qubits-k} of \Cref{alg:extensible} for $\m{K}'$, we search for all other kernels $\m{K}''$ with $\Call{ExtensibleQubits}{\m{K}'', i}=\Call{AllQubits}{}$ to be merged together with $\m{K}'$ at that time.

For example, after adding $g_7$ into $\m{K}_4$ in \Cref{fig:dp_with_optimization}, we create a singleton kernel $\m{K}_5$ for $g_8$. In the next iteration, we find that both $\m{K}_1$ and $\m{K}_5$ are subsumed by $g_9$, so we pick one arbitrarily to add $g_9$ into it. Suppose we add $g_9$ into $\m{K}_5$, then we will run line~\ref{extensible:qubits-k} of \Cref{alg:extensible} for $\m{K}_1$. Before running this line, we search for all other kernels with the extensible qubit set being all qubits -- $\m{K}_4$ and $\m{K}_5$. So we will either leave $\m{K}_1$ alone or merge it with $\m{K}_4$ or $\m{K}_5$, resulting in different $\KS{}$'s. In this particular example, merging $\m{K}_1$ with $\m{K}_5$ will be the best option.

%When merging multiple extensible kernels to generate a fixed kernel, \Sys restricts the maximum number of qubits for shared-memory kernels based on the GPU shared memory size and also sets a maximum number of qubits for fusion kernels where the cost will become too high otherwise.

%Recall that \Sys tracks the \kwins{} qubits for shared-memory kernels. To defer merging extensible kernels as far as possible, \Sys keeps multiple shared-memory kernels as extensible even if they share \kwins{} qubits. This optimization may require swapping adjacent gates that share a \kwins{} qubit, which will be described in the next paragraph.


%\ZJ{What is merging extensible kernels to generate fixed kernel?}\MX{See the paragraph "Deferring merging kernels".} \ZJ{What's a reasonable cost?} \MX{The cost function for kernels gives us the cost of fusion kernels for each number of qubits. When the number of qubits is too high, the cost can be prohibitive because it is proportional to two to the power of the number of qubits.}

\if 0
\ZJ{Old version <====================}
We have some other minor optimizations during the DP transition to reduce the number of DP states.

If a gate is subsumed by an existing kernel, we directly add the gate to that kernel without considering other choices.

If an existing extensible kernel is subsumed by a new gate (this may happen if the existing kernel consists of one gate and the new gate operates on all qubits in the existing gate and also some other qubits), we add the new gate to that kernel without considering other choices.

When merging extensible kernels to generate fixed kernels, we restrict the maximum size for shared-memory kernels, and also set a maximum size for fusion kernels based on a reasonable cost.

\ZJ{====================>}
\fi

\paragraph{Attaching single-qubit gates.}
Our preliminary experiments showed that the single-qubit gates of a quantum circuit could easily result in an exponential blowup in the number of DP states because of the independence between single-qubit gates applied to different qubits. To address this issue, we attach each single-qubit gate to an adjacent multi-qubit gate. If the single-qubit gate is \kwnonins{}, we mark the corresponding qubit \kwnonins{} in the attached gate. For single-qubit gates that are only adjacent to other single-qubit gates, we attach them together to the closest multi-qubit gate.


\paragraph{Post-processing}
After the DP algorithm, \Sys needs to merge some kernels together in $\KS{}$ before taking the cost as a post-processing step. 
Computing the minimum cost for merging kernels is NP-hard because the bin packing problem can be reduced to this problem.
\Sys uses a simple approximation algorithm that greedily packs the kernels in $\KS{}$, running in quasilinear time: (1) for fusion kernels, \Sys packs them towards the most cost-efficient density; (2) for shared-memory kernels, \Sys packs them towards the maximum shared-memory kernel size.

\paragraph{Pruning DP states.}
Another key optimization to reduce the DP states is {\em pruning}. A simple pruning based on the cost of the DP states would be suboptimal because we have not considered the cost of the kernels in $\KS{}$ which may contribute a lot.
%%%
%Because the number of DP states is still too high, we need to prune some of them during the DP. However, we cannot simply take the minimum cost among DP states because we have not considered the cost of the kernels which may contribute a lot.
During the DP, whenever the number of states at the same position $i$ in the circuit reaches a user-defined threshold $T$ at the beginning of an iteration (i.e., Line~\ref{dp:loop_i} in \Cref{alg:dp}), \Sys performs the post-processing step introduced above at the current position for all DP states and keeps $\frac{T}{2}$ DP states with the lowest cost after post-processing.
%we compute the ``kernel schedule at the end'' at the current position for each DP state to get the cost of kernels in $\KS{}$, and keep only the 1,000 DP states with the lowest total cost of kernels in $\KS{}$ and closed kernels.
This is the only optimization that may worsen the results. Our preliminary experimentation with this pruning suggested that it does not affect \Syss results. % \MX{I didn't do any experiment to back up this} \SC{I did it for 28-qft, treid 1000,2000,4000,8000, do we want to report it?}
We set $T = 500$ in our evaluation, which achieves good performance.



==> ilp_old.tex <==
\section{Hierarchical Circuit Partitioning}
\label{sec:partitioner}

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/state_vector_placement.png}
    \vspace{-1em}
    \caption{\Sys uses the aggregated DRAM of multiple nodes to store the state vector of a quantum system and sends state batches to GPUs for simulating quantum gates. A quantum simulation with $l$ logical, $r$ regional, and $o$ global qubits uses $2^o$ compute nodes, each of which stores $2^{l+r}$ states in the DRAM. Each batch includes $2^l$ states.}
    \label{fig:state_vector_placement}
\end{figure}


%\ZJ{We assume that logical qubits and physical qubits have already been defined before.}
To support scalable quantum circuit simulation that goes beyond GPU memory capacity, \Sys uses the aggregated DRAM of multiple nodes to store a state vector and processes the state vector on multiple GPUs in parallel in a batched fashion, as shown in \Cref{fig:state_vector_placement}.
%To avoid inter-device communication during the simulation of quantum gates, \Sys processes the state vector in a batched fashion where each gate can only access different states within the same batch.
%%%
%In addition, the state vector of a quantum simulation is partitioned across the DRAMs of different nodes. 
As a result, simulating the application of a gate may potentially involve inter-device and/or inter-node communications. Based on this observation, we divide physical qubits into three categories.

%\UA{The definition needs work. 1)  What is saved is the portion of the state, 2) the second half of each bullet would be best stated outside the definition.}
%\ZJ{How about the new definition?}

\begin{definition}[Local, regional, and global qubits]
\label{def:logical_regional_global}
For a quantum circuit simulation with $n$ qubits, let $q_i$ ($0\leq i \leq n-1)$ be the $i$-th physical qubit. Let each batch include $2^l$ states and let the DRAM of each node save $2^{l+r}$ states.
%We partition the qubits into a local, regional, and global subset such as each qubit belongs to exactly one of the three subsets:

\begin{itemize}

\item The first $l$ physical qubits (i.e., $q_0,...,q_{l-1}$) are {\em local} qubits.
    %Applying a quantum gate to a local simulation qubit only requires accessing states within a mini-batch and therefore avoids inter-device and inter-node communications.
\item The next $r$ physical qubits (i.e., $q_{l},...,q_{l+r-1}$) are {\em regional} qubits. 
    %Applying a quantum gate to a regional qubit requires accessing states in a different mini-batch but on the same node, and therefore only requires inter-device communications.
\item The final $o = n - l - r$ physical qubits (i.e., $q_{l+r},...,q_{n-1}$) are {\em global} qubits.
    %Applying a quantum gate to a global qubit requires inter-node communications.
\end{itemize}

\end{definition}

We categorize physical qubits into local, regional, and global subsets based on the communications required to simulate the application of a general quantum gate to these qubits.
First, applying a gate to a local qubit only requires accessing states within the same batch and therefore avoids communications.
Second, applying a gate to a regional qubit requires accessing states in different batches stored on the same compute node, which only requires inter-device (intra-node) communications.
Finally, applying a gate to a global qubit requires states stored on different compute nodes and thus involves inter-node commutations.

Given this partition of local, regional, and global qubits, we aim to map logical qubits of a circuit to physical qubits of \Sys's quantum circuit simulator in a way that avoids excessive communications.
To minimize the communication cost, we leverage a specific type of qubits, called {\em insular qubits}.
%
%To identify which gates may be included in a batch, and inspired by ``global gate specialization'' by H\"aner \emph{et~al.}~\cite{haner_05_2017}, we identify certain qubits of a gate as \kwins{}, which intuitively correspond to a qubit that may be considered local. \MX{I added a citation here, not sure if we want to mention it or not}

\begin{definition}[\Kwins{} Qubit]
\label{def:insular_qubit}
For a single-qubit gate, the qubit is \kwins if the
unitary matrix of the gate is diagonal or anti-diagonal, i.e., the
non-zero entries are along the (anti) diagonal.
%
For multi-qubit controlled-$U$ gates, all control qubits are \kwins\footnote{In some controlled-$U$ gates, any qubit can be chosen as the control qubit without changing the output. In such gates, all qubits are \kwins{}.}.
%For multi-qubit gates, we say that any control qubit of a (controlled) gate is \kwins{}.
%
All other qubits are \kwnonins{}.
\end{definition}

%\begin{wrapfigure}{r}{0.64\textwidth}
\begin{figure}
    \centering
    \vspace{-2em}
    \subfloat[Qubit remapping with inter\\-node communications.]{
    \includegraphics[scale=0.34]{figures/inter_node_communications.pdf}
    \label{fig:inter_node_communications}
    }
    \subfloat[Qubit remapping with inter\\-device communications.]{
    \includegraphics[scale=0.34]{figures/inter_device_communications.pdf}
    \label{fig:inter_device_communications}
    }
    \vspace{-1em}
    \caption{Communications for qubit remapping. The simulation has 1 local, 1 regional, and 1 global physical qubit. $p_i - q_j$ indicates that the $i$-th physical qubit is mapped to the $j$-th logical qubit. Inter-node communications are triggered if we change the mapping for global qubits (\Cref{fig:inter_node_communications}), and inter-device (intra-node) communications are triggered if we change the mapping for regional qubits (\Cref{fig:inter_device_communications}).}
    \label{fig:qubit_remapping}
%\end{wrapfigure}
\end{figure}


Our idea of \kwins{} qubits was inspired by {\em global gate specialization} introduced by H\"aner \emph{et~al.}~\cite{haner_05_2017}.
Intuitively, for a single-qubit gate with an \kwins{} qubit, computing each output state only depends on one input state (since the gate's unitary matrix is diagonal or anti-diagonal), which allows \Sys to map \kwins{} qubits to regional and/or global physical qubits without introducing any communications. This property allows \Sys to only consider the \kwnonins{} qubits of quantum gates when mapping qubits.

%Applying quantum gates to regional or global qubits introduces fine-grained inter-device and/or inter-node data transfers, resulting in significant communication overheads. 
%To address this issue, \Sys uses the batch processing approaches in modern ML systems and only applies gates to local qubits.
\Sys uses {\em qubit remapping} to adjust how logical qubits in a quantum circuit are mapped to physical qubits supported by \Sys.
%%%
\Sys's {\em circuit partitioner} splits a quantum circuit's simulation into multiple stages, each of which includes a subcircuit and uses a different mapping from logical to physical qubits.
%%%
Within each subcircuit, all \kwnonins{} qubits of all gates can only operate on \emph{local} physical qubits. 
This approach avoids any inter-device or inter-node communications within a stage and only requires all-to-all communications between stages to perform qubit remapping.


% \Sys uses a two-level approach to minimizing the communication cost of qubit remapping.
% First, a {\em high-level} circuit partitioner splits an input quantum circuit into disjoint subcircuits, each of which only includes gates whose \kwnonins{} qubits are mapped to {\em local and regional} qubits. 
% The goal of the high-level circuit partitioner is to minimize inter-node communications. 
% Second, a {\em low-level} circuit partitioner further splits each resulting circuit into disjoint subcircuits, each of which only includes gates whose \kwnonins{} qubits are mapped to {\em local} qubits.
% The low-level circuit partitioner minimizes inter-device communications.

% At the high level, the communication cost (i.e., amount of states transferred between different nodes during qubit remappings) depends on the number of swaps between global and non-global qubits. \Cref{fig:inter_node_communications} shows an example of qubit remapping that changes the mapping of the global qubit (i.e., $p_2$) from $q_2$ to $q_1$, which results in state transfers between compute nodes.
% %%%
% Similarly, at the low level, inter-device communications depend on the number of swaps between local and regional qubits. \Cref{fig:inter_device_communications} shows an example of qubit remapping that changes the mapping of a regional qubit (i.e., $p_1$) from $q_1$ to $q_0$, which results in state transfers between GPUs on the same node.

We formalize qubit remapping as a constrained optimization problem and design a binary integer linear programming (ILP) algorithm to discover a qubit remapping strategy that minimizes the total communication cost.

% \begin{problem}[Optimal qubit remapping]
% Given an inter-node communication cost factor $c$,
% %
% the optimal qubit remapping problem takes as input
% %
% a quantum circuit $\m{C}$, the number of local, regional, and global qubits $l, r, o$, and an integer $s$,
% %
% and returns at most $s$ stages $\m{C}_0,..., \m{C}_{s-1}$ that minimizes
% the total communication cost:
% \begin{equation}
% \sum_{i=0}^{s-2} (LocalSwaps + c \cdot GlobalSwaps)
% \label{eqn:ilp_objective_informal}
% \end{equation}

% such that each kernel consists of a contiguous segment of the gate sequence $\m{C}$.
% \label{problem:kernelization}
% \end{problem}

\paragraph{Qubit remapping problem.}
Given an inter-node communication cost factor $c$, for a given input circuit $\m{C}$ with $n$ qubits and $m$ gates and an integer $s$, \Sys's circuit partitioner splits $\m{C}$ into at most $s$ stages $\m{C}_0,..., \m{C}_{s-1}$ and determines a qubit mapping plan for each stage such that the \kwnonins{} qubits of all gates within a stage are mapped to local qubits. \Sys discovers a qubit remapping strategy that minimizes the total communication cost:
\begin{equation}
\sum_{i=0}^{s-2} \left(\Call{NumberOfLocalSwaps}{\m{C}_i, \m{C}_{i+1}} + c \cdot \Call{NumberOfGlobalSwaps}{\m{C}_i, \m{C}_{i+1}}\right),
\label{eqn:ilp_objective_informal}
\end{equation}
where $\Call{NumberOfLocalSwaps}{\m{C}_i, \m{C}_{i+1}}$ and $\Call{NumberOfGlobalSwaps}{\m{C}_i, \m{C}_{i+1}}$ are the number of \ZJ{TODO: define these two functions.}

Let $A_{q,k}$ and $G_{q,k}$ ($0\leq q < n$, $0 \leq k < s$) denote whether the $q$-th logical qubit is mapped to a local/global physical qubit at the $k$-th stage, and let $F_{g,k}$ ($0\leq g < m$, $0 \leq k < s$) denote if the $g$-th gate is finished by the end of the $k$-th stage. 
For each $A_{q,k}$ and $G_{q,k}$ ($k < s-1$), we also introduce two ancillary variables $S_{q,k}$ and $T_{q,k}$ that indicates whether there is a qubit swap associated with the $q$-th logical qubit between the $k$-th and $(k+1)$-th stages (i.e., $S_{q,k} =1$ if and only if $A_{q,k} = 0$ and $A_{q,k+1} = 1$; $T_{q,k} =1$ if and only if $G_{q,k} = 0$ and $G_{q,k+1} = 1$).
Note that $A_{q,k}$, $G_{q,k}$, $F_{g,k}$, $S_{q,k}$, and $T_{q,k}$ are all binary variables.
Minimizing the total cost of local-to-non-local and global-to-non-global swaps with constraints yields the following objective:

\begin{equation}
    \min \sum_{k=0}^{s-2} \sum_{q=0}^{n-1} \left(S_{q,k} + c \cdot T_{q,k}\right)\label{eqn:objective}
\end{equation}
subject to
\begin{align}
&A_{q,k+1}\leq A_{q,k} + S_{q,k} & \forall q \in [0,n-1]\ \ \forall k \in [0,s-2] \label{c1}\\
&G_{q,k+1}\leq G_{q,k} + T_{q,k} & \forall q \in [0,n-1]\ \ \forall k \in [0,s-2] \label{cdeft} \\
&F_{g,k}\leq F_{g,k+1} & \forall g \in \m{G}\ \ \forall k \in [0,s-2] \label{c2}\\
&F_{g, k}\leq F_{g,k-1} + A_{q,k} & \textrm{$q$ is a non-insular qubit of $g$}\label{c3}\\ 
&F_{g_1,k}\geq F_{g_2,k} & \forall (g_1, g_2) \in \m{E}\ \ \forall k \in [0,s-1]\label{c4}\\
&F_{g,s-1}=1 & \forall g \in \m{G} \label{c5} \\
&A_{q,k} + G_{q,k} \le 1 & \forall q \in [0,n-1]\ \ \forall k \in [0,s-1] \label{cag} \\
&\sum_{q=0}^{n-1}{A_{q,k}}=l & \forall k \in [0,s-1] \label{c6} \\
&\sum_{q=0}^{n-1}{G_{q,k}}=o & \forall k \in [0,s-1] \label{cglobal}
\end{align}

%\ZJ{FIXME: Shouldn't eqn 10 be $F_{g_1,k} \geq F_{g_2,k}$ since we need to execute $g_1$ before $g_2$?}
%\MX{Fixed and double-checked with the code}

We now describe these constraints. First, constraints~\ref{c1}, \ref{cdeft} and \ref{c2} can be derived from the definitions of $S_{q,k}$, $T_{q,k}$ and $F_{g,k}$. Second, constraint~\ref{c3} is a locality constraint that a gate $g$ can be executed at the $k$-th stage only if $g$'s non-insular qubits $q$ are all mapped to local physical qubits (i.e., $A_{q,k} = 1$).
Third, constraint~\ref{c4} represents a dependency constraint that all gates must be executed by following a topological order with respect to dependencies between them.
Fourth, constraint~\ref{c5} is derived from the completion constraint that all gates must be executed in the $s$ stages.
Next, constraint~\ref{cag} declares any qubit cannot be both local and global at the same time.
Finally, constraints~\ref{c6} and \ref{cglobal} specifies the hardware constraint that each stage has $l$ local physical qubits and $o$ global qubits.


\paragraph{ILP-based circuit partitioning.} For a given input circuit $\m{C}$ and an integer $s$ that specifies the maximum number of stages $\m{C}$ can be partitioned into, \Sys sends the objective (i.e., \Cref{eqn:objective}) and all constraints (i.e., \Cref{c1,cdeft,c2,c3,c4,c5,cag,c6,cglobal}) to an off-the-shelf integer-linear-programming (ILP) solver, which returns an assignment for matrices $A,G,F,S,T$ that minimizes the objective while satisfying all constraints. 
\Sys then partitions the input circuit $\m{C}$ into $s$ stages $(\m{C}_0,\m{M}_0),\dots,(\m{C}_{s-1},\m{M}_{s-1})$ based on $A$, $G$ and $F$, where $\m{C}_i$ is a subcircuit and $\m{M}_i$ is a qubit mapping.
Specifically, for a quantum gate $g \in \m{G}$, $g$ will be executed by the stage with index: $\min\{k | F_{g,k} = 1\}$. 
%%%
\Sys maps the $q$-th logical qubit to a local physical qubit at the $k$-th stage if $A_{q,k} = 1$, to a global qubit at the $k$-th stage if $G_{q,k} = 1$, and to a regional qubit if $A_{q,k} = G_{q,k} = 0$.

%\paragraph{Correctness of \Sys's circuit partitioning algorithm.} The correctness of \Sys's circuit partitioning algorithm is given by the combination of the following constraints. First, the dependency constraint~(\ref{c4}) guarantees that  \ZJ{explain the correctness of our ILP algorithm.} \MX{Do we need to explain? I think it's fine to delete this paragraph.}

%\paragraph{Two-level circuit partitioner.} 

Using the ILP solver as a subroutine, \Cref{alg:ilp} shows \Sys's circuit partitioning algorithm. The loop in line~\ref{ilp:loop_s} ensures that the number of stages is minimized in the function $\Call{Partition}{}$, and the ILP ensures that the total communication cost is minimized.
%, which allows \Sys to minimize inter-node communications in line~\ref{ilp:high_level}. Within each node, \Sys further minimizes inter-device communications (line~\ref{ilp:low_level}).

\begin{figure}[tb]
\small
\begin{algorithmic}[1]
% \Function{TwoLevelPartition}{$\m{C},l,r$}
% \State $\m{C}_0,\dots,\m{C}_{s-1} = \Call{Partition}{\m{C},l+r}$ \label{ilp:high_level}
% \For{$i=0,\dots,s-1$}
% \State $\m{C}_{i,0},\dots,\m{C}_{i,s_i} = \Call{Partition}{\m{C}_i,l}$\label{ilp:low_level}
% \EndFor
% \State \Return $(\m{C}_{0,0},\dots,\m{C}_{0,s_0}),\dots,(\m{C}_{s-1,0},\dots,\m{C}_{s-1,s_{s-1}})$
% \EndFunction
% \State
\Function{Partition}{$\m{C},l,o$}
\For{$s = 1, 2, \dots$} \label{ilp:loop_s}
\State $status, A, G, F = \Call{SolveILP}{\m{C},l,o,s}$
\If{$status = feasible$}
\State Find $(\m{C}_0,\m{M}_0),\dots,(\m{C}_{s-1},\m{M}_{s-1})$ based on $A$, $G$, $F$
\State \Return $(\m{C}_0,\m{M}_0),\dots,(\m{C}_{s-1},\m{M}_{s-1})$
\EndIf
\EndFor
\EndFunction
\end{algorithmic}
\vspace{-0.5em}
\caption{\Sys's circuit partitioning algorithm.\vspace{-0.5em}}
\label{alg:ilp}
\end{figure}

\begin{comment}
\section*{Old version}
\begin{definition}[Local, global, and mixed gates]
Given a partition of $n$ qubits, we say that


\begin{itemize}
\item a gate is local if it operates only on local qubits,

\item a gate is global if it operates only on global qubits,

\item and a gate is mixed if it operates both on global and local qubits.
\end{itemize}
\end{definition}

\begin{definition}[Benign gates]
  THIS NEEDS WORK
  
  These are global or mixed gates that can be ``executed'' locally and
  globally in an orthogonal fashion
  
\end{definition}

See also ``global gate specialization'' in \cite{haner_05_2017}.


We calculate the largest state vector size $2^\ell$ that each GPU can
hold including space for both input and output vectors.
%
We refer to $\ell$ as the number of local qubits.



Input: circuit and input state as an arbitrary state vector

Algorithm:

Determine the number of local and global qubits $\ell$ and $m = n - \ell$

Run ILP with the above parameters

ILP partitions the circuit into stages such that each stage has only
EXECUTABLE gates

For each stage do:
  Run the DP algorithm
  Perform


\ZJ{Motivate the necessity to do circuit partitioning; define this circuit partitioning problem; introduce the ILP algorithm}
Because we can only execute dense \MX{Define it somewhere} gates when they only operate on local qubits, we need to partition the circuit into several \emph{stages}, where each stage has a different set of local qubits. We will then execute the gates in the circuit stage by stage, and perform a qubit remapping between stages.

As the cost of qubit remapping is high, we use a 0-1 integer linear programming (ILP) approach to minimize the number of stages. When there are multiple solutions that minimize the number of stages, we want to find one to minimize the total number of local-global qubit pair swaps. The ILP is defined with the following variables:
\begin{itemize}
\item $a_{i,j} = 1$ iff the $i$-th qubit is a local qubit at the $j$-th stage,
\item $b_{i,j} = 1$ iff the $i$-th gate is finished before or at the $j$-th stage,
\item $s_{i,j} = 1$ iff $a_{i,j+1} = 1$ and $a_{i,j} = 0$, which is the number of local-global qubit pair swaps.
\end{itemize}

We iterate the number of stages $m$ to find the minimal one that has a feasible solution to the ILP:
\begin{align*}
&\text{Find } a_{i,j} \in \{0,1\}, b_{i,j} \in \{0,1\}, s_{i,j} \in \{0,1\} \\
&\text{that minimizes} \sum_{i,j} s_{i,j} \text{ (local-global qubit pair swaps)}\\
\text{s.t. }&\forall i, j, a_{i,j+1} \le a_{i,j} + s_{i,j} \text{ (definition of $s$)} \\
&\forall j, \sum_i a_{i,j} = k \text{ ($k$ local qubits per stage)} \\
&\forall i, j, b_{i,j} \le b_{i,j+1} \text{ (definition of $b$)}\\
&\forall i, j, \text{qubit }q\text{ of a dense gate }i, b_{i,j} - b_{i,j-1} \le a_{q,j} \\
& \text{\qquad (kernel execution requirement)} \\
&\forall j, \text{dependency edge }(i_1, i_2), b_{i_1, j} \ge b_{i_2, j} \\
& \text{\qquad (gate dependency requirement)} \\
&\forall i, b_{i,m} = 1 \text{ (we must have executed all gates at the end)}
\end{align*}

In this way, we find the local qubit sets at each stage as well as the gates executed at each stage to have the minimum total number of local-global qubit pair swaps on the basis of minimizing the number of qubit remappings.
\end{comment}


==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}

Quantum computing has established an advantage over classical
computing, especially in areas such as cryptography, machine learning,
and physical
sciences~\cite{nielsen2000quantum,bennett2020quantum,orus2019quantum,biamonte2017quantum,lloyd2013quantum,schuld2019quantum,aspuru2005simulated,babbush2015chemical}.
%
Several quantum computers have been built recently, including Sycamore~\cite{arute2019quantum}, Bristlecone, and Jiuzhang~\cite{zhong2020quantum}.
%
However, the robustness demands of many quantum applications exceed those
of modern {\em noisy intermediate-scale quantum} (NISQ) computers, which
suffer from decoherence and lack of error-correction~\cite{Preskill_2018, Corcoles_2020}.
%
Furthermore, NISQ computers are expensive resources---many remain inaccessible beyond a small group.
%
There has therefore been significant interest in quantum circuit simulation,
which enables performing robust quantum computation on classical parallel
machine.


A number of approaches to simulating quantum circuits have been proposed based
both on Schr\"odinger and Feynman's ideas, called state-vector and
Feynman-sums.
%
Even though approaches based on Feynman sums can require a small
amount of space, their time requirements appear exceedingly high and
therefore most modern simulators use Schroedinger-style or
state-vector quantum simulation.
%
%All approaches, however, suffer from an exponential space or time
%explosion problem due to the fundamentals of quantum computing.
%
%% A quantum system with $n$ quantum bits, called {\em qubits}, can be in a linear combination of $2^n$ basis states (roughly corresponding to $0, 1, \ldots,
%% 2^n-1$),
%% %
%% leading to exponential demand in the number of qubits on space and/or time.
%% %
%% Specifically, in popular {\em state-vector} based simulation (a.k.a., Schr\"odinger style simulation), tracking the state of a quantum system requires storing $2^n$ complex
%% numbers representing the linear combination of the $2^n$ basis states.

%% %% In a quantum system with $n$ {\em quantum} bits (called {\em qubits}),
%% %% we can entangle these qubits, which makes a quantum system in a
%% %% superposition of $2^n$ states.  The state of a quantum system can be
%% %% represented as a {\em state vector} consisting of $2^n$ complex
%% %% numbers.
%%
Several approaches have been proposed to tackle the scalability
challenges of state-vector simulation.
%
To improve performance, researchers exploit the plethora of
parallelism available in this task by using CPUs, GPUs, and parallel
machines~\cite{amariutei2011parallel, avila2014gpu,
avila2016optimizing, qiskit2019, gutierrez2010quantum, jones2019quest,
zhang2015quantum,smelyanskiy2016qhipster,suzuki2021qulacs,park_snuqs_2022,chen2021hyquas}.
%
To cope with the increasing demand of simulating larger quantum
circuits, recent work has proposed techniques for storing state
vectors on DRAM and secondary storage, including
disks~\cite{haner_05_2017,smelyanskiy2016qhipster}.
%
Even after over a decade of research, quantum circuit simulation
continues to remain challenging for performance and scalability.

At a high level of abstraction, there are three specific challenges to
state-vector simulation.
%
The first challenge is the scale.
%
The state vector for a simulation with $n$ qubits holds $2^n$ entries
called, amplitidutes, each of which is a complex number.
%
Even for modest values of $n$, storing and computing with this vector
becomes a challenge.
%
Second challenge is exploiting the paralellism, which is naturally
available, in quantum simulation.
%
Given a state vector, and a gate in a quantum circuit, we can compute
the impact of applying that gate to the state, by appyling the gate to
each and every amplitude of the state vector in parallel.
%
Given that the state vector is large, this approach yields large
amounts of parallelism but this parallelism is very fine grained,
because a gate usually represents a small amount of computation.
%
The third challenge is the communication costs that arise due to large
amount of memory that must be accessed for applying each and every
gate.
%
These communication costs can become especially dominant, because,
being large, most simulators must store the state vector by
distributing among the available nodes of the underlying architecture
used for simulation.


In this paper, we 

the cost of communication inherent to quantum
computing.
%
Applying

%
At a high level of abstraction, this may seem trivial: in a quantum
circuit simulation, a gate may be applied to each and every element of
the state ver




In this paper, we propose techniques for improving the performance and scale of quantum circuit simulation by taking advantage of modern GPU systems, especially those designed for machine learning, at three different scales: small, medium, and large.
%Some of our techniques are inspired by and build on top of recent development of machine learning (ML) systems.
%

\begin{itemize}
\item At the {\em large} scale of multiple compute nodes, we propose techniques to minimize inter-node communications by partitioning a quantum circuit into multiple subcircuits, each of which is simulated on a node without inter-node communications. The idea is to limit all inter-node communications to occur between stages and pack all computation inside the stages.

\item At the {\em medium} scale of multiple GPU devices on a single node,  we
  propose techniques\xupeng{which techniques? there are ``three'' techniques here, its better to have some titles or section references to help people to distinguish these three techniques for three scales} to minimize inter-device communication between devices by
  partitioning the node's circuit into subcircuits each of which can be simulated in a single GPU
  in isolation. The idea is to limit all inter-device communication to occur between batches and pack all computation inside the batches.
  
\item At the {\em small} scale of a single GPU, we propose techniques for
  performant simulation by formulating the
  \emph{kernelization problem} of partitioning the GPU's circuit subcircuits each of which can be simulated efficiently by a GPU kernel.
\end{itemize}
%
%Taken together, this approach ensures performance and scalability by making good use of modern GPU hardware, at multiple scales.
%

We ground this multi-scale approach by identifying key challenges, formulating them into specific optimization problems, and solving these problems by using a combination of algorithmic and systems techniques.

%
To minimize communication cost at the medium scale\xupeng{It is confusing to start from medium scale, rather than large scale}, we observe that it
is possible to simulate a subcircuit on a single GPU if all possible states of the 
subcircuit fit
into that GPU's memory.
%
Based on this observation, we can partition a quantum circuit into
smaller subcircuits, each of which can be simulated in a ``batch'' by
operating on a small, local (to GPU)  set of states, without
communicating with other GPUs.
%
To do this partition optimally, we formulate the problem of
determining the batches as constraint problem that can be solved by an
Integer Linear Program (ILP), and thus by existing ILP solvers.
%
To minimize communication at the large scale, 
%
We realize that we can use the same technique (as in the medium scale) and minimize
communication between multiple nodes in a GPU cluster by dividing the
quantum circuits into subcircuits, each of which can be simulates in a
``stage'' by operating on a small, \emph{regional} or ``node-local'',
set of states, without communicating with other nodes.
%


%The idea behind this approach is to create tight clusters of local,
%intense computation interspersed by data movement that sends the
%needed data to where it will be used.

Our medium and large scale techniques minimize communication and tightly pack computation into sections\xupeng{Here is the first time we use ``section'', it is better to explain this abstraction, especially the difference with subcircuits} that ultimately take place on a GPU somewhere in the system.
%
To take maximum advantage of each GPU, we exploit the plethora of data parallelism in 
quantum simulation.
%
Even though at the limit, each gate can be applied to all of the
states in parallel, this approach can lead to
parallelism that is too fine-grained to be advantageous unless all
data fits in a GPU's ``shared memory''.
%
We therefore coarsen\xupeng{The causal relationship here is confusing, try to rewrite, why we mention shared memory, why too fine grained} the available parallelism by considering two methods, one based of
replacing a set of gates by a single matrix-vector multiplation
operation (it is straightforward to compute the specific matrix by
quantum-computing knowledge)\xupeng{it is not ``starightforward'', we need to mention the background in one sentence before, e.g., the third paragraph of Intro?} and the other by using GPU shared
memory and applying each gate independently.
%
We then propose a dynamic programming algorithm for partitioning a
circuit into a subcircuits each of which can be optimally executed by
kernel performing the two coarsening methods.


These techniques were inspired by recent advances in machine learning
(ML) systems~\cite{Tensorflow, pytorch, jia2019flexflow, zheng22-alpa}
that enable fast and performant ML computations on modern GPUs by
leveraging  parallelism at multiple scales.
%
We build \xupeng{add a few words to describe \Sys here, e.g., a distributed quantum circuit simulation system \Sys over GPU clusters on top of a multi-GPU DL system FlexFlow}\Sys on top of FlexFlow~\cite{jia2019flexflow}, a distributed
multi-GPU system for DNN training.
%
Overall, instead of building an ``end-to-end'' quantum circuit simulator that directly
maps quantum computation to GPU instruction set architectures (ISAs),
we leverage the fact that both quantum circuit simulation and ML computation
rely heavily on tensor algebra operations and use recent advances on
machine learning to develop a performant and scalable quantum
simulator.\xupeng{For me with a mlsys background, I feel like its better to talk about the similarities on tensor algebra operations before parallelism}

To evaluate our approach, we use a variety of quantum circuits as
benchmarks and simulate them on up to 64 GPUs across 16 nodes.
%
Our experimental results show that \Sys is up to 7.3$\times$ faster than state-of-the-air GPU-based simulators and can scale to large quantum circuits that go beyond GPU memory capacity. 
For example, \Sys can simulate a 32-qubit quantum circuit on one \SI{16}{GB} NVIDIA V100 GPU, while simulating this circuit on existing GPU-based simulators would require 16 such GPUs.

In summary, this paper makes the following contributions.

\begin{itemize}
\item An approach to fast and scalable quantum circuit simulation that
  optimizes for communication and computations costs at multiple
  levels of scale.

    \item An ILP algorithm to minimize inter-device communications in
      quantum circuit simulation.
    \item A dynamic programming algorithm for optimal kernelization
      and to maximize single-GPU efficiency in quantum circuit
      simulation.
    \item A quantum circuit simulator built on top of an ML system that outperforms existing GPU-based simulators by up to 7.3$\times$.
    %\item Empirical results on a GPU cluster that shows the performance and scalability benefits of the proposed techniques.
\end{itemize}


\section{Introduction}
\label{sec:intro}

Quantum computing has established an advantage over classical
computing, especially in areas such as cryptography, machine learning,
and physical
sciences~\cite{nielsen2000quantum,bennett2020quantum,orus2019quantum,biamonte2017quantum,lloyd2013quantum,schuld2019quantum,aspuru2005simulated,babbush2015chemical}.
%
Several quantum computers have been built recently, including Sycamore~\cite{arute2019quantum}, Bristlecone~\cite{bristlecone}, and Jiuzhang~\cite{zhong2020quantum}.
%
However, the robustness demands of many quantum applications exceed those
of modern {\em noisy intermediate-scale quantum} (NISQ) computers, which
suffer from decoherence and lack of error-correction~\cite{Preskill_2018, Corcoles_2020}.
%
Furthermore, NISQ computers are expensive resources---many remain inaccessible beyond a small group.
%
There has therefore been significant interest in quantum circuit simulation,
which enables performing robust quantum computation on classical parallel
machine.


A number of approaches to simulating quantum circuits have been proposed based
both on Schr\"odinger and Feynman's ideas, called state-vector and
Feynman-sums.
%
All approaches, however, suffer from an exponential space or time
explosion problem due to the fundamentals of quantum computing.
%
A quantum system with $n$ quantum bits, called {\em qubits}, can be in a linear combination of $2^n$ basis states (roughly corresponding to $0, 1, \ldots,
2^n-1$),
%
leading to exponential demand in the number of qubits on space and/or time.
%
Specifically, in popular {\em state-vector} based simulation (a.k.a., Schr\"odinger style simulation), tracking the state of a quantum system requires storing $2^n$ complex
numbers representing the linear combination of the $2^n$ basis states.

%\UA{We want to be more specific here.  I will think about it... I think we want to be more constructive.}

To address the scalability challenge posed by quantum circuit simulation, modern simulation systems use DRAM and/or disks to store a state vector and simulate quantum circuits on CPUs~\cite{haner_05_2017,smelyanskiy2016qhipster}.
However, this approach does not take advantage of the increasingly common GPU resources on modern hardware platforms.
Recent work has introduced a variety of GPU-based simulators that either only use GPUs on a single node or achieve suboptimal performance and limited GPU utilization for  simulation across nodes due to fine-grained inter-node communications and very low arithmetic intensity of quantum circuit simulation~\cite{chen2021hyquas, li2021svsim}.

On the other hand, recent advances in machine learning (ML) systems~\cite{Tensorflow, pytorch, jia2019flexflow, zheng22-alpa} enable fast and performant ML computations on modern GPUs and leverage efficient parallelization strategies to distribute ML computations across GPUs on today's hardware platforms. 

In this paper, we present a new approach to realizing fast and scalable quantum circuit simulation on modern GPU clusters. 
Instead of building an ``end-to-end'' quantum simulation system that directly offloads simulation's computation to GPU instruction set architectures (ISAs), we leverage an important observation that both quantum circuit simulation and ML computation revolve around tensor algebra operations such as matrix multiplication, and build \Sys, a system that enables fast and scalable quantum simulation by transforming a quantum circuit simulation to ML computations and parallelizing simulation across multiple GPUs on an ML system.
This approach allows \Sys to directly benefit from existing ML systems techniques to accelerate quantum circuit simulation.
Achieving performant simulation on an ML system requires addressing two key challenges.

\paragraph{Challenge \#1.} Simulating the application of a quantum gate to one or multiple qubits involves strided accesses to the state vector, which requires {\em fine-grained} inter-node and inter-GPU communications. 
However, most ML systems leverage independence between training samples and use {\em data parallelism} to partition samples across GPUs, which avoids any communications during the forward processing and backward propagation of a training iteration while only performs communications between iterations.
%use data parallelism to partition ML computations across nodes and only perform coarse-grained inter-node communications between training iterations.

To eliminate fine-grained communications and align with the communication pattern of modern ML systems, \Sys uses {\em qubit remapping} to dynamically adjust how logical qubits in a quantum circuit map to physical qubits supported by \Syss simulation system.
\Syss {\em circuit partitioner} splits an input circuit into disjoint stages, within each of which quantum gates only operate on the physical qubits whose computation does not require inter-device or inter-node communication. 
This design eliminates any data transfers within a stage and only requires an all-to-all communication between stages, which is effectively supported by modern ML systems.
%%%
To minimize the cost of all-to-all communications, we formalize qubit remapping as a constrained optimization problem, and design a binary integer linear programming (ILP) algorithm to discover an optimal qubit remapping strategy for an arbitrary quantum circuit.

\paragraph{Challenge \#2.} Quantum circuit simulation generally has much lower arithmetic intensity compared to ML operations. For example, recent work reported an arithmetic intensity of less than 0.5 for simulating real-world quantum circuits~\cite{haner_05_2017}. 
%\MX{This (page 3, lower left corner in their paper) is not related to simulating a 45-qubit quantum circuit -- it is simply analyzing the work for the state-vector approach, assuming read from memory and write back for each gate. I would say "A straightforward implementation has an arithmetic intensity of less than 0.5, which suggests quantum simulation is memory-bandwidth bound~\cite{haner_05_2017}." then motivate by memory-bandwidth bound.}
%%%
To improve simulation performance on GPUs, \Syss {\em circuit kernelizer} assigns individual gates of a stage to GPU kernels while minimizing the overall execution time
of these kernels.
%\xupeng{It this achieved by better GPU utilization?} \ZJ{Yes and reduced GPU memory accesses}
%\ZJ{TODO: need to mention operation fusion in ML systems and difference between it and circuit kernelization.}
We formalize circuit kernelization as an optimization problem and propose a dynamic programming algorithm to maximize simulation performance on modern GPUs.

We built \Sys on top of a distributed multi-GPU ML system (i.e., FlexFlow~\cite{jia2019flexflow}). Our evaluation on a variety of quantum
circuits on up to 64 GPUs (on 16 nodes) shows that \Sys
is up to 7.3$\times$ faster than state-of-the-art GPU-based simulators and can scale to large quantum circuits that go beyond GPU memory capacity. For example, \Sys can simulate a 32-qubit quantum circuit on one \SI{16}{GB} NVIDIA V100 GPU,
while simulating this circuit on existing GPU-based simulators requires 16 such GPUs.

In summary, this paper makes the following contributions.

\begin{itemize}
    \item An approach to fast and scalable quantum circuit simulation by transforming it to ML computations and running it on an ML system.
    \item An ILP algorithm to optimize qubit remapping by minimizing inter-device communications in quantum circuit simulation.
    \item A dynamic programming algorithm to solve the circuit kernelization problem.
    \item A quantum circuit simulator built on top of an ML system that realizes our techniques and outperforms the best existing GPU-based simulators by 2.0$\times$ on average (7.3$\times$ at most).
\end{itemize}


==> overview.tex <==
\if 0
\section*{Overview and Terminology}
\ZJ{To be removed <=======}
We consider a heteregenous multi-node GPU architecture,
%
where
%
each node has a DRAM (dynamic RAM) module shared by multiple GPUs.
%
We assume for simplicity that the architecture is uniform: any node
has the same memory and clock speed as any other node and any GPU has the same memory and clock speed as any other GPU.
%
We assume that the nodes are connected with a interconnect network
allowing any two to communicate.
%

We refer the term \defn{local} to refer to properties of GPUs,
\defn{regional} to refer to properties of nodes, and \defn{global} to
refer to properties across multiple nodes and their GPUs.

At a high level, the idea behind our approach to efficient and
scalable simulation is
%
to partition the computation into local, regional, and global
components and ensure that the bulk of the computation is local, and
then regional, and rarely global.
%
To partition the computation, we consider the quantum circuit input to
our simulator and refer to its qubits as \defn{logical qubits}.
%
We then map each logical qubit to a \defn{simulation qubit} which is in turn map to a local GPU, a regional node, or the global system as a whole.
%

Throughout the paper, we use $n$ to refer to the total number of
logical qubits in the circuit (to be simulated).
%
We assume that GPU memory size is a power of two and define $\ell$ as
binary logarithm of the GPU memory size.
%
Similarly we assume that node memory size is a power of two and define
$r$ as the binary logarithm of the node memory size.
\ZJ{To be removed =======>}
\fi 
